ParaLiNGAM: Parallel Causal Structure Learning for Linear non-Gaussian Acyclic Models

One of the key objectives in many fields in machine learning is to discover causal relationships among a set of variables from observational data. In linear non-Gaussian acyclic models (LiNGAM), it can be shown that the true underlying causal structure can be identified uniquely from merely observational data. DirectLiNGAM algorithm is a well-known solution to learn the true causal structure in high dimensional setting. DirectLiNGAM algorithm executes in a sequence of iterations and it performs a set of comparisons between pairs of variables in each iteration. Unfortunately, the runtime of this algorithm grows significantly as the number of variables increases. In this paper, we propose a parallel algorithm, called ParaLiNGAM, to learn casual structures based on DirectLiNGAM algorithm. We propose a threshold mechanism that can reduce the number of comparisons remarkably compared with the sequential solution. Moreover, in order to further reduce runtime, we employ a messaging mechanism between workers and derive some mathematical formulations to simplify the execution of comparisons. We also present an implementation of ParaLiNGAM on GPU, considering hardware constraints. Experimental results on synthetic and real data show that the implementation of proposed algorithm on GPU can outperform DirectLiNGAM by a factor up to 4600 X.

==> LiNGAM(A23) - arXiv/alg.tex <==
\section{ParaLiNGAM}
\label{sec:alg}

In this section, we present the ParaLiNGAM algorithm for accelerating computationally-intensive part of DirectLiNGAM without changing its accuracy.

As mentioned before, DirectLiNGAM discovers causal order in $p$ iterations. Moreover, these iterations are consecutive, i.e., an iteration cannot be started unless the previous has been already finished. Herein, ParaLiNGAM is also executed in $p$ iterations. \mRefFig{fig:alg:base} illustrates the procedure of one iteration.
\begin{figure*}[tp]
	\centering
	\includegraphics[width = \textwidth]{fig/flowchart}	
	\caption{Procedure of one iteration in ParaLiNGAM: Each iteration is divided into steps.
	Each step has three parts: Compare, Message Passing, Scheduler, which are accomplished with pre-selected workers from the previous step ($\mathcal{W}_k$). Details are discussed in Section \ref{sec:alg}.}
	\label{fig:alg:base}
\end{figure*}


In each iteration, computations of each variable are assigned to a specific \textbf{worker}. Iterations are broken into \textbf{steps}. In each step $k$, a subset of all workers($\mathcal{W}$) in an iteration, which is denoted by $\mathcal{W}_k$, is selected to start comparing themselves with other workers (Compare part). Next, the workers inform each other about their computations by sending messages (Message Passing part).
Finally, the \textbf{scheduler} gathers all workers' scores and selects some of the workers for the next step, i.e., $\mathcal{W}_{k+1}$. 

\begin{algorithm}%[tp]
	\begin{algorithmic}[1]
		\Input $\mathcal{X}$
		\Output $K$
		%
		\State $K=\emptyset$
		\State $U =[1,\cdots, p]$
		\State Par: $NormalizeData(\mathcal{X})$
		\State Par: $ \Sigma = CalculateCovMat(\mathcal{X})$
		\Repeat
			\State Par: $root = ParaFindRoot(\mathcal{X}, U, \Sigma)$
			\State Append $root$ to $K$
			\State Remove $root$ from $U$
			\State Par: $\mathcal{X} = UpdataData(\mathcal{X}, U, \Sigma, root)\hfill//$Sec\ref{sec:math}
			\label{line:RegressRoot}
			\State Par: $\Sigma = UpdateCovMat(\mathcal{X}, U, \Sigma, root) \hfill//$ Sec\ref{sec:math}
			\label{line:UpdateCovMat}
		\Until{$U$ is not empty}
	\end{algorithmic}
	\caption{ParaLiNGAM} 
	\label{alg:ParaLiNGAM}
\end{algorithm}

The description of ParaLiNGAM is given in \mRefAlg{alg:ParaLiNGAM}. The lines starting with ``Par" show that they are executed in parallel. ParaLiNGAM algorithm is executed similar to DirectLiNGAM. First, we initialize $U$ and $K$ (lines $1-2$). Next, we find a casual order in lines $5-11$. General procedure of this algorithm is same as DirectLiNGAM, however, computations' details have been changed which we discuss them in the sequel.

In DirectLiNGAM, samples of all variables have to be normalized in $FindRoot$ function (lines $7-8$ in \mRefAlg{alg:baseLiNGAM_FR}). For sake of efficiency, all variables are normalized simultaneously in line $3$ of \mRefAlg{alg:ParaLiNGAM} for the first iteration. For the next iterations, this task is done with $UpdateData$ function (line $9$ in \mRefAlg{alg:ParaLiNGAM}).

Regressing variables on each other, is a frequent task in DirectLiNGAM which is performed in $Compare$ (lines $9-10$ in \mRefAlg{alg:baseLiNGAM_FR}) and $RegressRoot$ (line $7$ in \mRefAlg{alg:baseLiNGAM}) functions, and it needs variables' covariance matrix. Hence, it is desirable to store covariance matrix (which we denote it by $\Sigma$) in each iteration to avoid redundant computations. In \mRefAlg{alg:ParaLiNGAM}, the first covariance matrix of variables is calculated in line $4$, and it is updated in each iteration (line $10$). 
Furthermore, we will show in Section \ref{sec:math} how to reuse computations from previous iterations in normalizing data and obtaining the covariance matrix which results in reducing the computational complexity without degrading the accuracy.
 
 % As mentioned before, ParaLiNGAM changes not only computations' order in DirectLiNGAM {\color{red} Where did you talk about it?} but also its procedure without degrading its accuracy (More details in \mRefSec{sec:math}).

We discussed the summary of changes in \mRefAlg{alg:baseLiNGAM}. Now, we are ready to explain these changes in more details. First, we present a parallel solution for finding root in each iteration ($ParaFindRoot$ function in Algorithm \ref{alg:ParaLiNGAM_FR}).

\begin{algorithm}%[tp]
	\begin{algorithmic}[1]
		\Input $\mathcal{X}, U, \Sigma$
		\Output $root$
		\item[\textbf{\# of Workers:}] $|U|$
		%
		\If {$U$ has only one element}
			\State return the element
		\EndIf
		\State $r = |U|$
		\State $\mathcal{W} = [1, 2, 3, ..., r]$
%		// still needs some changes \red{what do you mean?}
		\State $\mathcal{S} = [\textbf{0}]_{r}$
		\State $\mathcal{M} = [\emptyset]_{r\times r}$
		\State $\mathcal{D} = diag([True]_r)$
%		\State $\mathcal{E} = \textbf{0}_{r\times r}\hfill//$Sec \ref{sec:compare}
%		\State $\mathcal{B} = [False]_{r\times r}\hfill//$Sec \ref{sec:compare}
		\State $State = \{U, \Sigma, r, \mathcal{S}, \mathcal{M}, \mathcal{D}, \gamma \}$
		\State $\mathcal{W}' = \mathcal{W}$
		\State $\mathcal{C} = \textbf{1}_{r}$
		\Repeat
		
%		//Perform lines $15-16$ with $ \mathcal{W}'$ workers in parallel \blue{Since we have defined the parallel notation, shall we use it again? Par:}
%			\ForAll {$ w \in \mathcal{W}'$}
				\State Par: $\mathcal{S}[w] += Compare(w, \mathcal{C}[w], State)$%\hfill//$Sec\ref{sec:compare}
				\State Par: $\mathcal{S}[w] += CheckMessages(w, State)\hfill//$Sec\ref{sec:messaging}
%			\EndFor
			\State $finished, \mathcal{W'}, \mathcal{C} = Scheduler (\mathcal{W},  \mathcal{C}, State)\hfill//$Sec\ref{sec:scheduler}
		\Until{$finished == True$}
		\State $root=U[\arg\min(\mathcal{S})]$
	\end{algorithmic}
	\caption{$ParaFindRoot$} 
	\label{alg:ParaLiNGAM_FR}
\end{algorithm}

In order to find root in DirectLiNGAM (\mRefAlg{alg:baseLiNGAM_FR}), all variables compare themselves with other ones (line $5$). In the parallel version, we assign each variable to a worker to perform its computations. In other words, instead of a $for$ statement in line $5$ of \mRefAlg{alg:baseLiNGAM_FR}, we have workers, which can work in parallel to perform the comparisons. Moreover, comparing each variable/worker to other variables/workers is divided into steps instead of iterating on all variables (line $6$ \mRefAlg{alg:baseLiNGAM_FR}). Next, we discuss the details of presented solution for finding root (\mRefAlg{alg:ParaLiNGAM_FR}).

The description of $ParaFindRoot$ function is given in  \mRefAlg{alg:ParaLiNGAM_FR}. First, we define $r$ as the number of remaining variables in this iteration, which equals to the size of $U$ (line $4$). In each iteration, every pair of variables have to be compared to find the root. Moreover, these comparing procedure is independent of each other. We can use $r$ workers, and worker $i$ is responsible for performing variable $U[i]$'s computations.
For simplicity of notations, from now on, we denote workers by the corresponding variables assigned to them. We define $\mathcal{W}$ as a list of all workers' indices in an iteration (line $5$). In line $6$,  $\mathcal{S}$ is initialized the same as the main algorithm (line $4$ in \mRefAlg{alg:baseLiNGAM_FR}) to store scores. Each worker might have useful information for the other workers, which can be shared with a \textbf{messaging} mechanism. To do so, we define $\mathcal{M}$ which is $r\times r$ matrix filled with $\emptyset$ (line $7$). Worker $i$ can send a message to worker $j$ by writing in $\mathcal{M}[j][i]$. More details of the messaging mechanism and its effect on the performance of algorithm will be discussed in \mRefSec{sec:messaging}. Note that matrix $\mathcal{M}$ is just temporary memory for messaging and it resets in each step. 
Hence, another variable is required for evaluating the progress of an iteration.
%to store the status of iteration and the status is utilized in several tasks such as selecting the active workers for the next step. 
%Status of iteration can be specified with comparisons are finishes or remained by each worker {\color{red} What do you mean here?}.
For this purpose, in line $8$, we define a $r \times r$ matrix $\mathcal{D}$ in which diagonal entries are initially $True$ while others are $False$, to monitor workers' progress. Worker $i$  writes $True$ in $\mathcal{D}[i][j]$ after comparing itself with worker $j$.
%In lines $9-10$, required variables in comparing procedure are defined. More details about comparing two workers and also the mentioned variables are given in \mRefSec{sec:compare} \red{correct it!}.
For sake of brevity, we collect all variables defined in Algorithm \ref{alg:ParaLiNGAM_FR}, and the threshold $\gamma$ with a small value (Section \ref{sec:thresh}, \ref{sec:scheduler}) in set $State$ (line $9$).

As mentioned before, finding root in each iteration is divided into steps. In each step, some workers are selected, and each of them has to compare itself to another worker. Selected workers are indicated with $\mathcal{W}'$ (line $10$). In the first step of each iteration, all of workers have same priority. Hence, $\mathcal{W}'$ equals $\mathcal{W}$. Moreover, list of target workers to be compared with is defined as $\mathcal{C}$ (line $11$), and worker $i$ compares itself with $\mathcal{C}[i]$. At the beginning of each iteration, $\mathcal{C}$ is initiated with a list filled with $1$, which means all of the workers start comparing themselves with the first worker.

In each step, first, selected workers compare themselves with the assigned workers and send a message (line $13$). Comparing and sending a message is an independent task for each worker and can be performed in parallel. Then, workers check for new messages from others and update their scores (line $14$). Afterwards, $Scheduler$ selects workers for the next step according to this step's status. Moreover, it modifies $\mathcal{C}$ for selected workers (line $15$) and determines whether to terminate an iteration after checking its $State$. Finally, similar to \mRefAlg{alg:baseLiNGAM_FR}, the worker with minimum score is chosen as the root of iteration (line $17$). 

There are still some implementation details that will be discussed in the next parts. More specifically, 
messaging between workers will be discussed in \mRefSec{sec:messaging}. The details of \textbf{threshold} mechanism which determines $\mathcal{W}'$, the set of selected workers, is given in \mRefSec{sec:thresh}. The scheduling of workers based on the threshold mechanism is discussed in \mRefSec{sec:scheduler}. Mathematical simplification for accelerating $UpdateData$ and $UpdateCovMat$ process is also discussed in \mRefSec{sec:math}. Finally, implementation of this algorithm on GPU and further details on some parts of solution are given in \mRefSec{sec:alg2}.

\subsection{Messaging}
\label{sec:messaging}
In DirectLiNGAM, as mentioned in \mRefSec{sec:baseLiNGAM}, computation of test $\mTest$ for $x_i \rightarrow x_j$ has some similarities to the ones for $x_i \leftarrow x_j$. It is worth mentioning, this property is not just for $\mTest$, and this technique can be used for some other tests \cite{hyvarinen2013pairwise}.
When worker $i$ compares itself to worker $j$ (computing $\mTest(x_i, x_j, r_i^{(j)}, r_j^{(i)})$), it can also compute the test in the reverse direction ($\mTest(x_j, x_i, r_j^{(i)}, r_i^{(j)})$), which is worker $j$'s task. Hence, we can assign full comparison to just one worker, and after finishing each comparison, the worker who performed the test, has to inform the other worker about its result by sending a message. With messaging, which does not add computation load
%(details in \mRefSec{sec:compare}) \red{correct it},
we can halve the comparisons (from $p(p-1)$ to $p(p-1)/2$). To use this mechanism, every active worker in a step has to send a message after finishing its comparison (line 13 in \mRefAlg{alg:ParaLiNGAM_FR}), and each worker checks for their messages (which can be from any $r-1$ other workers in the whole iteration) with $CheckMessages$ function.

\begin{algorithm}%[tp]
	\begin{algorithmic}[1]
		\Input $w, State$
		\Output $score$
		%
		\State $score = 0$
		\For{$~~(i=1;~~ i <= r;~~ i+=1)$}
			\If{$\mathcal{M}[w,i] != \emptyset$}
				\State $score += \mathcal{M}[w, i]$
				\State$\mathcal{D}[w, i] = True$
				\State $\mathcal{M}[w, i] = \emptyset$
			\EndIf
		\EndFor
			
	\end{algorithmic}
	\caption{$CheckMessages$}
	\label{alg:CheckMessages}
\end{algorithm}

The description of $CheckMessages$ function is given in \mRefAlg{alg:CheckMessages}. First, we define $score$ as variable for sum of scores. In lines 2-3, worker $w$ checks for new messages. If another worker, say $i$, has sent a message, first, $score$ is updated (line 4). Next, worker $w$ marks the sender worker ($i$) as "done" by writing $True$ in $\mathcal{D}[w, i]$ (line 5). Finally, message is replaced with $\emptyset$ to prevent it from recalculation in next steps. The senders and receivers might not be active simultaneously in one step. As a result, workers consider messages from whole workers in an iteration and not just from active workers in the current step.

\subsection{Threshold}
\label{sec:thresh}
As mentioned earlier, we need to perform $p(p-1)/2$ comparisons in each iteration. However, all of them are not necessary. Suppose that the final score of the root in an iteration is $0.05$. In this case, we can terminate any worker's computation whose score has reached $0.05$.
To reduce the number of comparisons, we consider an upper bound for the score which we call it threshold, and assume that root's score will probably be less than this threshold. If that is the case, the iteration is over and we can choose the root when at least one worker could finish its comparisons without reaching the threshold, while all other workers reach it without completing their tasks. 

Herein, the main issue is how to choose a proper threshold.
To overcome this issue, first, we choose a small value for the threshold. Furthermore, we terminate workers who have already reached this value. Then, if all workers terminate and neither of them could finish their comparisons, we increase the threshold. We continue this procedure till iteration termination conditions satisfy, i.e., at least one worker finish all their comparisons without reaching the threshold. Consequently, using the threshold mechanism can result in reducing the number of comparisons.
%
%Consequently, using a threshold mechanism would split an iteration into some steps where in each step, we might increase the threshold that we used in the previous step. \blue{would determine some variables, which we can neglect their comparisons in the steps}

Now, we discuss the correctness of the threshold mechanism in each iteration.
At the end of each iteration, each worker is in one of these two groups:
1) Worker's score is more than the threshold, and it may not even finish its comparisons.
2) Worker finishes its comparisons, and still, its score is below the threshold.
Workers in the first group have higher scores than the threshold even they continue their comparisons. The root is a worker with a minimum score. As a result, it is always chosen from the second group of workers. In fact, we select the root from workers in the second group which has the minimum score among them. Hence, early termination of the first group of workers does not affect algorithm results.
Details of reducing number of comparisons by the threshold mechanism are discussed in \mRefSec{sec:scheduler}.


\subsection{Scheduler}
\label{sec:scheduler}

In this part, we explain how to schedule workers with the threshold mechanism. At the end of each step, the scheduler has to decide whether or not to finish current iteration.


\begin{algorithm}%[tp]
	\begin{algorithmic}[1]
		\Input $\mathcal{W}, \mathcal{C}, State$
		\Output $finish, \mathcal{W'}, \mathcal{C}$
		%
		\State $finish = False$
		\ForAll {$ w \in \mathcal{W}$} // checking the termination 
			\If{$\mathcal{S}[w] < \gamma$}
					\If {$\mathcal{D}[w,:]$ has at least one $False$}
						\State $finish = False$
						\State \textbf{Break}
					\Else
						\State $finish = True$
					\EndIf
			\EndIf	
		\EndFor
		\If {$finish$}
			\State \textbf{return}
		\EndIf
		\While{$\mathcal{S}[w] > \gamma, ~~ \forall w \in \mathcal{W}$} 
			\State $\gamma = \gamma \times c$ // updating threshold
		\EndWhile
		\State $\mathcal{W'} = [ w \in \mathcal{W}~~|~~ \mathcal{S}[w] < \gamma]$
%		\State $\mathcal{C} = [0]_{|\mathcal{W}|}$
		\ForAll {$ w \in \mathcal{W'}$}
			\Repeat
				\State $\mathcal{C}[w] += 1$
			\Until{$(\mathcal{D}[w,\mathcal{C}[w]] == False ~~ \& \& ~~ \mathcal{C}[\mathcal{C}[w]]!=w) ~~ | | ~~ \mathcal{C}[w] > |\mathcal{W}| $}
		\EndFor
		\State $\mathcal{W'} = \mathcal{W'}\backslash[ w \in \mathcal{W'}~~|~~ \mathcal{C}[w] > |\mathcal{W}|]$	
		
	\end{algorithmic}
	\caption{$Scheduler$}
	\label{alg:Scheduler}
\end{algorithm}

As mentioned earlier in \mRefSec{sec:thresh}, if at least one worker has finished its comparisons and its score is below than the threshold, we can terminate the iteration.

The description of scheduler is given in \mRefAlg{alg:Scheduler}. The termination of an iteration is checked in lines $1-14$. First, we define $finish$ as a flag for termination conditions (line $1$). Then, we have to find workers with scores less than the threshold (line $2-3$) and check whether they have finished their comparisons or not (line 4). If at least one worker has unfinished comparisons and its score is below than the threshold, we need to continue another step (lines $5-6$). If some workers have finished their comparisons, $finish$ is changed to $True$, and we wait for other workers' status (line $7-9$). Then, we check $finish$ value and decide whether or not to terminate the iteration (lines $12-14$).

Now we discuss the scheduler's task when an iteration is not terminated and it should be continued for another step. For the new step, we have to change threshold if it is needed (lines $15-17$). There are multiple ways to increase the value of threshold. Here, we just multiply by some constant $c$ (see \mRefSec{sec:schGPU} for more details on selecting the desirable constant $c$). We continue updating threshold until at least one of workers' scores is below than the threshold. Then, the scheduler chooses workers ($\mathcal{W}'$) and comparison targets ($\mathcal{C}$) for the next step.


Workers with scores less than the threshold are considered as the workers of new step (line $18$). $\mathcal{C}$ is updated for the selected workers in lines $19-23$. As mentioned, $\mathcal{C}$ is initialized with \textbf{$1$} and workers need to compare themselves with worker $1$ for their first step. For the next steps, we start increasing $\mathcal{C}[w]$ for worker $w$ till we find a pair ($w$, $\mathcal{C}[w]$) which their comparison has not performed yet.
In a step, it might occur that two workers compare with each other  simultaneously, which is not desirable as they are performing redundant tests. In order to prevent these cases, the scheduler also checks for repetitive pairs of comparison (second condition in line $22$).

A worker might finish its comparisons while its score was greater than the threshold, but it becomes smaller after updating threshold. Such workers have to wait for the next step. In this case, first, $\mathcal{C}[w]$ is set to a value greater than $|\mathcal{C}|$, then the scheduler omits such workers from $\mathcal{W}'$ (line $24$).

Some details of scheduling depend on implementation considerations and will be discussed in \mRefSec{sec:schGPU}.


\subsection{Mathematic Simplification}
\label{sec:math}

As mentioned earlier, DirectLiNGAM algorithm always works with normalized data. Furthermore, normalization and regression tasks are frequently performed in the algorithm. These tasks depend on computing the covariances of variables, and it would be desirable to obtain them in an efficient manner. In this section, we demonstrate that if the relationship between variables is linear, which is one of the main assumption in LiNGAM, we can estimate variance of residual of regressions and use them in normalization step (lines $7 - 8$ in \mRefAlg{alg:baseLiNGAM_FR}). Furthermore, we can estimate coefficients used in regressing variables in data updating procedure (line $7$ in \mRefAlg{alg:baseLiNGAM}).

First, we calculate  the adjusted sample variance $s^2$ for residual of a regression. Residual of $x_i$ regressed on $x_j$ (denoted by $r_i^{(j)}$) is defined as:
\begin{equation}
r_i^{(j)} = x_i - \frac{cov(x_i, x_j)}{var(x_j)} x_j, i \neq j.
\end{equation}
Moreover, if we assume that samples are normalized, it can be shown that $E[r_i^{(j)}] = 0$. Furthermore, calculating residuals only needs the covariance matrix. Consider  $b = cov(x_i, x_j)$ and assume that both variables are normalized. We can write:
\begin{equation}
	\begin{split}
	s^2 &= \frac{1}{n-1} \sum (r_i^{(j)} - E[r_i^{(j)}])^2 \\
	&= \frac{1}{n-1} \sum (x_i - b x_j)^2 = \frac{1}{n-1} \sum (x_i^2 - b^2x_j^2 - 2b x_i x_j) \\
	&= \frac{1}{n-1} (\sum x_i^2 + b^2 \sum x_j^2 - 2b\sum x_i x_j) \\
	&= var(x_i) + b^2 var(x_j) - 2b cov(x_i, x_j)\\
	&= 1 + b^2 - 2b^2 = 1 - b^2 = 1 - cov^2(x_i, x_j).
	\end{split}
	\label{eq:var_update}
\end{equation}

Thus, we showed that the variance of $r_i^{(j)}$ is equal to $1 - cov^2(x_i, x_j)$. Therefore, in order to normalize it, we just have to divide all samples to $\sqrt{1 - cov^2(x_i, x_j)}$. The details of $UpdateData$ function, which is called in \mRefAlg{alg:ParaLiNGAM}, is given in \mRefAlg{alg:UpdateData}.
\begin{algorithm}%[tp]
	\begin{algorithmic}[1]
		\Input $\mathcal{X}, U, \Sigma, root$
		\Output $\mathcal{X}$
		\item[\textbf{\# of Workers:}] $|U|$
%		\ForAll {$ w \in \mathcal{W}'$}
		\State $\mathcal{W} = [1, 2, 3, ..., |U|]$
		
%		Perform lines $2-4$ with $ \mathcal{W}$ workers in parallel
%		
%		\blue{Par: syntax}
%		 \For {$~~(i=0;~~ i < |\mathcal{X}[w,:]|;~~ i+=1)$}
%			\State $\mathcal{X}[w, i] = \dfrac{\mathcal{X}[w, i] - \Sigma[w, root] \mathcal{X}[root, i]}{\sqrt{1 - \Sigma^2[w, root]}}$
%		\EndFor
%		
%		\blue{I could not write Par: before the "for" command by the algnewcommand, so I did it manually. Is it ok?}
		\State Par: \textbf{for} {$~~(i=0;~~ i < |\mathcal{X}[w,:]|;~~ i+=1)$} \textbf{do}
			\State $~~~~\mathcal{X}[w, i] = \dfrac{\mathcal{X}[w, i] - \Sigma[w, root] \mathcal{X}[root, i]}{\sqrt{1 - \Sigma^2[w, root]}}$
		\State \textbf{end for}
	\end{algorithmic}
	\caption{$UpdateData$} 
	\label{alg:UpdateData}
\end{algorithm}

Next, we calculate the covariance between two residuals, which can be used in computing the covariance matrix for the next iteration.
Suppose we have $b_1 = cov(x_i, x_{root})$ and $b_2 = cov(x_j, x_{root})$. We have:
\begin{equation}
	\begin{split}
	cov(r_i^{root}, r_j^{root}) &= \frac{1}{n-1} \sum (x_i - b_1x_{root})(x_j - b_2x_{root}) \\
	&= \!\begin{multlined}[t]
		\frac{1}{n-1} \sum (x_ix_j - b_2x_ix_{root}  - b_1 x_j x_{root} \\+ b_1b_2x_{root}^2)
	\end{multlined}\\
	&= \!\begin{multlined}[t]
		cov(x_i, x_j) - b_2 cov(x_i, x_{root}) \\- b_1 cov(x_j, x_{root}) + b_1b_2 var(x_{root})
	\end{multlined}\\
	&= cov(x_i, x_j) - b_1b_2.
	\end{split}
	\label{eq:CovUpdate}
\end{equation}
From Equations \ref{eq:CovUpdate} and \ref{eq:var_update}, we can simply update the covariance matrix in each iteration just from the covariance matrix in the previous iteration, without using variables' samples (excluding the first iteration).
Details of $UpdateCovMat$ Function, which is called in \mRefAlg{alg:ParaLiNGAM}, is given in \mRefAlg{alg:UpdateCovMat}. Please note that $r_i^{root}$ and $r_j^{root}$ are not normalized in \mRefEq{eq:CovUpdate}. Therefore, it is needed to divided the expression for the covariance by the variances of  $r_i^{root}$ and $r_j^{root}$ (line 3 in \mRefAlg{alg:UpdateCovMat}).


\begin{algorithm}%[tp]
	\begin{algorithmic}[1]
		\Input $\mathcal{X}, U, \Sigma, root$
		\Output $\Sigma$
		\item[\textbf{\# of Workers:}] $|U|$
%		\ForAll {$ w \in \mathcal{W}'$}
		\State $\mathcal{W} = [1, 2, 3, ..., |U|]$
		
%		\ForAll {$ j \in U$}
%			\State $\Sigma[w, j] = \dfrac{\Sigma[w, j] - \Sigma[w, root] \Sigma[j, root]} {\sqrt{1 - \Sigma^2[w, root]}\sqrt{1 - \Sigma^2[j, root]}}$
%		\EndFor
%		
%		\blue{I could not write Par: before the "for" command by the algnewcommand, so I did it manually. Is it ok?}
		\State Par: \textbf{for} {$~~(i=0;~~ i < |\Sigma[w,:]|;~~ i+=1)$} \textbf{do}
			\State $~~~~\Sigma[w, j] = \dfrac{\Sigma[w, j] - \Sigma[w, root] \Sigma[j, root]} {\sqrt{1 - \Sigma^2[w, root]}\sqrt{1 - \Sigma^2[j, root]}}$
		\State \textbf{end for}
	\end{algorithmic}
	\caption{$UpdateCovMat$} 
	\label{alg:UpdateCovMat}
\end{algorithm}

%This section presents our proposed solution for acceleration of the computationally-intensive portion of DirectLiNGAM algorithm. Steps of this algorithm are sequential, but in each step, we can perform tests of each variable in parallel. In this section, first, we introduce the messaging method for saving computations and reusing them, in \mRefSec{sec:msg}. Then, we discuss how we can parallelize the DirectLiNGAM and balance the work of each worker in \mRefSec{sec:par}. Then, we introduce a threshold method to early termination of workers and saving computation in \mRefSec{sec:thresh}. We use mathematical simplification for accelerating data update process, which is discussed in \mRefSec{sec:math}. The solution is implemented on GPU using CUDA parallel programming API. Furthermore, A short background on CUDA is presented in \mRefAlg{sec:cuda}, and the ParaLiNGAM is introduced in \mRefSec{sec:ParaLiNGAM}. Further details on some parts of the proposed solution are discussed later in \mRefSec{sec:alg2}.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Messaging}
%\label{sec:msg}
%In DirectLiNGAM, the test $\mTest$ has symmetry and calculation of $\mTest$ for $x_i \rightarrow x_j$ has similarities to $x_i \leftarrow x_j$. It is worth mentioning, this property is not just for $\mTest$, and this technique can be used for most tests. These similarities means that with excess calculations in $\mTest(x_i, x_j, r_i^{(j)}, r_j^{(i)})$ (while  computing scores for $x_i$), we can calculate $\mTest(x_j, x_i, r_j^{(i)}, r_i^{(j)})$ which is belongs to $x_j$ variable. We can store these scores to reuse them in calculation of other variables. To do so, we propose a Messaging procedure, and each variable calculates both ways causal scores( $x_i \rightarrow x_j$ and $x_i \leftarrow x_j$) and sends other one a message to let it know it does not need to calculate this test again. In ParaLiNGAM, we send a message after accomplishing a comparison. In order to check for new messages, we use $UpdateScore$ function, which gathers all of new scores in messages received from other variables.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Working in Parallel}
%\label{sec:par}
%In \mRefAlg{alg:baseLiNGAM}, in each step, each variable has to compare itself to others, and calculations of variables are independent of other variables. For simplicity, we call each comparison a \textbf{task}, and we can do these tasks in parallel.
%\begin{figure}[tp]
%	\centering
%	\includegraphics[width = \columnwidth]{fig/parLiNGAM}	
%	\caption{An execution of ParaLiNGAM on \mRefEx{ex:base}. Squares and circles indicate works and tasks. Also, the arrows illustrate the order of tasks done by corresponding worker.}
%	\label{fig:pre:parLiNGAMex} 
%\end{figure}
%See the left side of \mRefFig{fig:pre:parLiNGAMex}, which is workflow of parallel execution of DirectLingam algorithm for \mRefEx{ex:base}. Suppose we have $W=5$ workers and name them $w_i, 1 \leq i \leq W$, which each of them is going to do $x_i$'s tasks. We can also assume that all workers start their tasks simultaneously. Because of messaging between variables, only green colored tasks are necessary. Moreover, two tasks connected via blue line have exact computations, and both send messages together. Also, we avoid it via a lock mechanism(further details in \mRefSec{sec:alg2}). As we see, load of each worker in naive implementation is not equal, and $w_1$ exits and finishes its tasks after the first level of tasks due to messages it will receive from other workers, but $w_5$ has to complete all of its tasks alone till the end. To overcome this problem, we have to balance the load of each worker. We can do this by giving an order of tasks. For example, if each worker starts comparing itself with the next index of variables (the right side), then each worker has to do same amount of tasks. This ordering also reduces the probability of collision between workers, in which both variables do the same task. However, in practice, all workers do not work at same speed, so the lock mechanism is still necessary.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Threshold}
%\label{sec:thresh}
%In base version of the algorithm (\mRefSec{sec:baseDL}), every variable is compared to all of the other variables. If we knew the score of root and say it was going to be less than $0.1$, at some point we could tell for sure that $x_1$(after performing the second task(comparison) with $x_2$) is not the root and terminate it to save computation. However, we cannot predict the score of the root, unless we perform all tasks. But, we can define a threshold $\gamma$ with a small value and terminate computation of variables in which their score exceeds the threshold. However, all variables may be terminated too, and still, no one is chosen for the root. For this matter, we can update the threshold value and continue the calculations of each variable, till one of them finishes its tasks without hitting the threshold again. In practice, updating threshold and continuing a process has overhead, and we can not act too greedy about it. Consider \mRefFig{fig:pre:parLiNGAMex}, red lines indicate termination of calculations because score of the variable reaches the threshold $\gamma = 0.1$, not to mention $x_3$ is the root of step $1$ and completes all of its tasks without reaching the threshold. It may seem that reordering used in previous section is pointless because we use locks and may terminate a worker, and most of variables are not going to finish their tasks anyway. However, the point of reordering is that we always perform tasks for new information in the beginning of work. We indeed use the lock mechanism, but it is not free and has overhead, and it is more efficient to prevent it as much as we can.
%
%In the main solution, to check the threshold we use $EarlyTermination$ function, which compares score of a variable with the threshold. We use this function in two places; first, at beginning of one variable's computation, which is terminated before, and we want to continue it. Second, after completing a task, which we have just updated the score of a variable and want to check if we have reached the threshold or not.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Mathematical simplification}
%\label{sec:math}
%As we see in \mRefAlg{alg:baseLiNGAMGPU}, algorithm always work with normalized data. Furthermore, normalization and regression are calculations used in the algorithm repeatedly. These calculations depend on variance and covariance of variables, and it would be more efficient if we could somehow estimate them. We show that if model strictly follows the linear model, which is a basic assumption in LiNGAM, we can estimate variance of residual of regressions, and use them in normalization step(lines 11, 12 in \mRefAlg{alg:baseLiNGAM_FR}). Furthermore, we can estimate coefficients used in regressing data used in data updating procedure(line 7 in \mRefAlg{alg:baseLiNGAM}).
%
%First, we calculate  the adjusted sample variance $s^2$ for residual of a regression. Residual of $x_i$ regressed on $x_j$ (donated by $r_i^{(j)}$) is defined as 
%\begin{equation}
%r_i^{(j)} = x_i - \frac{cov(x_i, x_j)}{var(x_j)} x_j (i \neq j).
%\end{equation}
%Also, if we suppose that samples are normalized, which means that variance of all variables is one and $E[r_i^{(j)}] = 0$. As a result, to regress two variables, we only need their covariance. Consider  $b = cov(x_i, x_j)$ and both variables are normalized, we can write
%\begin{equation}
%	\begin{split}
%	s^2 &= \frac{1}{n-1} \sum (r_i^{(j)} - mean(r_i^{(j)}))^2 \\
%	&= \frac{1}{n-1} \sum (x_i - b x_j)^2 = \frac{1}{n-1} \sum (x_i^2 - b^2x_j^2 - 2b x_i x_j) \\
%	&= \frac{1}{n-1} (\sum x_i^2 + b^2 \sum x_j^2 - 2b\sum x_i x_j) \\
%	&= var(x_i) + b^2 var(x_j) - 2b cov(x_i, x_j)\\
%	&= 1 - b^2 + 2b^2 = 1 - b^2 = 1 - cov^2(x_i, x_j).
%	\end{split}
%	\label{eq:var_update}
%\end{equation}
%
%So it is proven that variance of $r_i^{(j)}$ is equal to $1 - cov^2(x_i, x_j)$ and we can use it normalizing residuals.
%
%Next, we are going to calculate covariance between two residuals. The covariance matrix for new step consists of covariance of residual of variables regress on the previous step's root. Suppose we have $b_1 = cov(x_i, x_{root})$ and $b_2 = cov(x_j, x_{root})$, then we can write
%\begin{equation}
%	\begin{split}
%	cov(r_i^{root}, r_j^{root}) &= \frac{1}{n-1} \sum (x_i - b_1x_{root})(x_j - b_2x_{root}) \\
%	&= \!\begin{multlined}[t]
%		\frac{1}{n-1} \sum (x_ix_j - b_2x_ix_{root}  - b_1 x_j x_{root} \\+ b_1b_2x_{root}^2)
%	\end{multlined}\\
%	&= \!\begin{multlined}[t]
%		cov(x_i, x_j) - b_2 cov(x_i, x_{root}) \\- b_1 cov(x_j, x_{root}) + b_1b_2 var(x_{root})
%	\end{multlined}\\
%	&= cov(x_i, x_j) - b_1b_2
%	\end{split}
%	\label{eq:covUpdate}
%\end{equation}
%So with these two equations, we can estimate the coefficients for the whole of the algorithm only by using covariance information gathered from the beginning of algorithm. More details of their usage is discussed in \mRefSec{sec:ParaLiNGAM}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{CUDA}
%\label{sec:cuda}
%% main text is obtained from cuPC paper
%So far we have talked about some aspects of the solution. In these two sections, we are going to discuss the implementation of it on CUDA which is a parallel programming API for Nvidia GPUs. GPU is a massively parallel processor with hundreds to thousands of cores. 
%%
%CUDA follows a hierarchical programming model. At the top level, computationally intensive functions are specified by the programmer as CUDA \textbf{kernels}. A kernel is specified as a sequential function for a single \textbf{thread}. The kernel is then launched for parallel execution on the GPU by specifying the number of concurrent threads. 
%
%Threads are grouped into \textbf{blocks}. A kernel consists of a number of blocks, and every block consists of a number of threads. 
%%
%Every block has access to a small, on-chip and low-latency memory, called \textbf{shared memory}. The shared memory of a block is accessible to all threads within that block, but not to any thread from other blocks.
%
%In order to identify blocks within a kernel, and also, threads within a block, a set of indices are used in the CUDA API, for instance, $blockIdx.x$ as the block index in dimension $x$ within a kernel, and $threadIdx.x$ as the thread index in dimension $x$ within a block. There are other dimensions in CUDA, but for brevity, we only use them and denote these two indices as $bx$ and $tx$, respectively.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{ParaLiNGAM}
%\label{sec:ParaLiNGAM}
%\begin{algorithm}[tp]
%	\begin{algorithmic}[1]
%		\Input $\mathcal{X}$
%		\Output $K$
%		%
%		\State $K=\emptyset$
%		\State $U =\{1,\cdots, p\}$
%		\State GPU: $NormalizeData(\mathcal{X})$
%		\State GPU: $ \Sigma = CalculateCovMat(\mathcal{X})$
%		\Repeat
%			\State $root = ParaFindRoot(\mathcal{X}, U, \Sigma)$
%			\State Append $root$ to $K$
%			\State Remove $root$ from $U$
%			\State GPU: $RegressRoot(\mathcal{X}, U, \Sigma, root)$
%			\State GPU: $UpdateCovMat(\mathcal{X}, U, \Sigma, root)$	
%		\Until{$U$ is not empty}
%	\end{algorithmic}
%	\caption{DirectLiNGAM Opt Version} 
%	\label{alg:baseLiNGAMGPU}
%\end{algorithm}
%
%
%\begin{algorithm}[tp]
%	\begin{algorithmic}[1]
%		\Input $\mathcal{X}, U, \Sigma$
%		\Output $root$
%		%
%		\State $\gamma = 1e-7 $
%		\If {$U$ has only one element}
%			\State return the element
%		\EndIf
%		\State $\mathcal{C} = [1, 2, ..., p]$
%		\State $\mathcal{S} = \textbf{0}_{p}$
%		\State $\mathcal{SA} = \textbf{0}_{p\times p}$
%		\State $\mathcal{E} = \textbf{0}_{p\times p}$
%		\State $\mathcal{M} = [False]_{p\times p}$
%		\State $\mathcal{B} = [False]_{p\times p}$
%		\State $\mathcal{D} = [False]_{p\times p}$
%		\State $finish = False$
%		\Repeat
%			\State GPU: $finish, \mathcal{S}, \mathcal{M}, \mathcal{C}, \mathcal{SA}, \mathcal{E}, \mathcal{B},
%			\mathcal{D} = DoAll(\mathcal{X}, U, \Sigma, \gamma, \mathcal{S}, \mathcal{M}, \mathcal{C}, \mathcal{SA}, \mathcal{E}, \mathcal{B},
%			\mathcal{D})$
%%TODO check this line after renaming variables
%%TODO we can write like below ...
%%			\State GPU: DoAll(\mathcal{X}, U, \Sigma, \gamma, Scores, \mathcal{M}, \mathcal{C}, finish)$
%			\State $\gamma *= 10$
%		\Until{$finish$}
%		
%		\State $root=$ index of minimum element in $\mathcal{S}$
%	\end{algorithmic}
%	\caption{$ParaFindRoot$} 
%	\label{alg:baseLiNGAM_FR_GPU}
%\end{algorithm}
%
%
%%\begin{algorithm}[tp]
%%	\begin{algorithmic}[1]
%%		\Input $\mathcal{X}, U, \Sigma, \gamma, \mathcal{S}, \mathcal{M}, \mathcal{C}$
%%		\Output $finish, \mathcal{S}$
%%		\Block p
%%		\Thread $512$ 
%%		\State $dim = U[bx] $
%%		\State Load $\mathcal{C}$ and $\mathcal{S}$ from previous run
%%		\State $UpdateScore(\mathcal{S}[dim], \mathcal{M}[dim])$
%%%TODO check the code
%%		\State $EarlyTermination(\mathcal{S}[dim], \gamma)$
%%		%\State $CalculateEntropy(X[dim])$ if has not calculated yet
%%		\State $j = Next(\mathcal{C}[dim])$
%%		\Repeat
%%			\State $Compare(x_{dim}, x_j, \Sigma)$
%%			\State $UpdateScore(\mathcal{S}[dim], \mathcal{M}[dim])$
%%			\State $EarlyTermination(\mathcal{S}[dim], treshold)$
%%%TODO check the code
%%			\State $j = Next(\mathcal{C}[dim])$
%%		\Until{$j != dim$}
%%		\State $CheckAll()$
%%		
%%%		\If {all of compares are done}
%%%			\State $UpdateScore(\mathcal{S}[dim], \mathcal{M}[dim])$
%%%			\State $finish = True$
%%%		\Else
%%%			\State Store $\mathcal{C}$ and $\mathcal{S}$
%%%		\EndIf
%%	\end{algorithmic}
%%	\caption{$Do All$} 
%%	\label{alg:DOALL_GPU}
%%\end{algorithm}
%
%\begin{algorithm}[tp]
%	\begin{algorithmic}[1]
%		\Input $\mathcal{X}, U, \Sigma, \gamma, \mathcal{S}, \mathcal{M}, \mathcal{C}$
%		\Output $finish, \mathcal{S}, \mathcal{M}, \mathcal{C}, \mathcal{SA}, \mathcal{E}, \mathcal{B}, \mathcal{D}$
%		\Block p
%		\Thread $512$ 
%		\State shared: $cntr$
%		\State $BrkFlag = False$
%		\State $dim = U[bx] $
%		\State $id = tx $
%		\State $temp = 0$
%		\For{$~~(j=id;~~ j < size(U);~~ j=j+512)$}
%			\If {$\mathcal{M}[dim][j]$} \label{alg:cuPC:E:if}
%				\State $temp+= \mathcal{SA}[dim][j]$
%				\State $\mathcal{M}[dim][j] = False$
%				\State $\mathcal{D}[dim][j] = True$
%			\EndIf
%		\EndFor
%		\State th0: $Score = Reduce(temp) + \mathcal{S}[dim]$
%		\If {$Score > \gamma$}
%			\State Return
%		\EndIf
%		
%		\Repeat
%			\State th0: $cntr = (U[\mathcal{C}[dim]]+1)\%size(U)$
%		\Until{$\mathcal{D}[dim][cntr]$ is $False$}
%		\Repeat
%			\State $Compare(dim, cntr)$
%			\State exactly same lines 5..12
%			\If {$Score > \gamma$}
%				\State $BrkFlag = True$
%			\EndIf
%			\Repeat
%				\State th0: $cntr = (U[\mathcal{C}[dim]]+1)\%size(U)$
%			\Until{$\mathcal{D}[dim][cntr]$ is $False$}
%		\Until{$counter != dim$}
%		\If {$BrkFlag$}
%			\State th0: $\mathcal{C}[dim] = cntr$
%		\Else
%			\For{$~(j=0;~~ j < size(U);~~ j=j+1)$}
%				\If {$!\mathcal{D}[dim][j] \& i != bx$} 
%					\While{$!\mathcal{M}[dim][j]$}
%					\EndWhile
%					\State th0: $Score += \mathcal{SA}[dim][i]$
%				\EndIf
%			\EndFor
%			\State th0: $finish = True$
%		\EndIf
%		\State th0: $\mathcal{S}[dim] = Score$
%	\end{algorithmic}
%	\caption{$Do All$} 
%	\label{alg:DOALL_GPU_all}
%\end{algorithm}
%
%\begin{algorithm}[tp]
%	\begin{algorithmic}[1]
%	\If {$U[\mathcal{C}[dim]] == dim ~~ \&\& ~~ !CalcDone[dim][dim]$}
%		\State $\mathcal{E}[dim][dim] = Entropy(dim,dim)$
%		\State th0: $CalcDone[dim][dim] = True$
%	\EndIf
%		\State $ind1 = min\{dim, cntr\}$
%		\State $ind2 = max\{dim, cntr\}$
%		\If {$!CalcDone[ind1][ind2]$}
%			\If {$! \mathcal{B} [ind1][ind2]$}
%				\State th0: $\mathcal{B} [ind1][ind2] = True$
%				\State $\mathcal{E}[dim][cntr] = Entropy(dim,counter)$
%				\State $\mathcal{E}[cntr][dim] = Entropy(cntr,dim)$
%				\State th0: $CalcDone[ind1][ind2] = True$
%				\State th0: $\mathcal{B} [ind1][ind2] = True$
%			\Else
%				\State th0: $cntr = (U[\mathcal{C}[dim]]+1)\%size(U)$
%				\State \textbf{continue}
%			\EndIf
%		\EndIf
%		\If {$!CalcDone[cntr][cntr]$}
%			\State $\mathcal{E}[cntr][cntr] = Entropy(cntr,cntr)$
%			\State $CalcDone[cntr][cntr] = True$
%		\EndIf
%		\State th0: $result = \mathcal{E}[cntr][cntr] + \mathcal{E}[dim][cntr] - (\mathcal{E}[dim][dim] + \mathcal{E}[cntr][dim])$
%		\If {$result < 0$}
%			\State th0: $Score += result^2$
%		\Else
%			\State th0: $\mathcal{SA}[cntr][dim] = result^2$
%		\EndIf
%		\State th0: $\mathcal{D}[dim][cntr] = True$
%		\State th0: $\mathcal{M}[cntr][dim] = True$
%	\end{algorithmic}
%	\caption{$Do All$} 
%	\label{alg:DOALL_GPU_all}
%\end{algorithm}
%
%
%
%%TODO extra
%%talking about Done matrix
%The main part of algorithm is similar to main algorithm(\mRefSec{sec:baseDL}), first, we normalize data on GPU(line 3). Then, we calculate covariance matrix $\Sigma$ once for all, and for the rest of algorithm we only estimate $\Sigma$ (line 11) using \mRefEq{eq:covUpdate}. Then, we use \mRefAlg{alg:baseLiNGAM_FR_GPU} in order to find the root. For updating data procedure, we use $RegressRoot$ function which uses coefficients from $\Sigma$ to regress variables on root, moreover, we normalize residuals by \mRefEq{eq:var_update}.
%%TODO extra
%%we can explain more detail about calculations and GPU functions
%
%See \mRefAlg{alg:baseLiNGAM_FR_GPU}. First we define threshold $\gamma$ and set it to a small value(line 1). Furthermore, we define $\mathcal{C}$ set, which $\mathcal{C}[i]$ indicates the variable that $x_i$ is going to compare itself to. As explained in \mRefSec{sec:par} in order to balance the load of workers, default value of $\mathcal{C}[i]$ is $i+1$.
%$\mathcal{S}$ is defined same as \mRefAlg{alg:baseLiNGAM_FR}.
%Then, we define set of $p$ empty sets $\mathcal{M}$, where $\mathcal{M}[i]$ is inbox for $x_i$, and other variables write corresponding messages in it. We use these three sets to save algorithm state to restore it in case that all of variables are terminated by reaching the threshold. The $finish$ flag indicates if any variable has finished its tasks without hitting threshold. If $finish$ returned false, we have to update it. Various strategies can be employed to update threshold by using prior knowledge from data and threshold's behavior in previous steps. However, for generality, we update it by multiplying to 10(line10). In order to perform all calculations, we use the $DoAll$ function.
%%TODO extra
%%talk about scores and messages [i]
%
%See \mRefAlg{alg:DOALL_GPU}. Tasks of each variable can be run in parallel (\mRefSec{sec:par})).So, we use $p$ blocks. Moreover, in each block, we use 512 threads to handle computations.
%%TODO extra
%%can explain more if needed. However, GPU has a hardware limitation in the count of simultaneously running blocks. Number of threads is dependent on hardware, sample size,...
%In each variable, first, we define $dim$, the id of a variable, which the block is going to compute.
%Then, we check for $dim$'s previous run state(line 2) and update its score by messages it has received so far(line 3). Then, we check its score(line 4) to determine it has already reached the threshold or not. Now that we are sure about threshold, we do comparisons. Next variable to compare is determined by $Next$ function. It returns first index after $\mathcal{C}[dim]$ where $dim$ still has not received a message from(it has not been computed yet). Also, it locks the comparison so that $x_j$ can skip this computation. Next, we compare $x_dim$ with $x_j$(line 7). More details about comparison procedure is in \mRefSec{sec:alg2}. After comparison, we check for new messages and threshold. 
%% we can check time to time 
%Next, we update $j$ index for next comparison.
%When $j$ reaches $dim$ it means we have already checked all of variables, or other variables will do the remaining comparisons and send the result. At last, we use $CheckAll$ function in order to picked up remaining messages and check the threshold if $dim$ has new messages and score is updated.


==> LiNGAM(A23) - arXiv/exp.tex <==
\section{Experimental Evaluation}
\label{sec:exp}

\subsection{Setup}
\label{sec:exp:setting}

The proposed ParaLiNGAM algorithm is implemented in C++ language using CUDA parallel programming framework. The source code is available online \cite{sourceParaLiNGAM}. 

We experimentally evaluate ParaLiNGAM, along with DirectLiNGAM \cite{shimizu2011directlingam} which is a sequential method. The latest implementation of DirectLiNGAM is in Python language \cite{sourceDirectLiNGAM}. In order to have fair comparisons, we re-implemented DirectLiNGAM in C++ language. This implementation is available in \cite{sourceParaLiNGAM}. 

%TODO
% may be a python wrapper

We employ a server machine with Intel Xeon CPU with $16$ cores operating at $2.1$ GHz. 
%
Since DirectLiNGAM is a sequential method, it is executed on a single core.
%
The CUDA kernels in ParaLiNGAM are executed on Nvidia Tesla V$100$ GPU, and the other procedures are executed sequentially on a single core. We use Ubuntu OS 20.04, GCC version 9.3, and CUDA version 11.1.



\subsection{Real-World Datasets}
\label{sec:exp:real_data} 


\begin{table}[tp]
	\centering
	\caption{Benchmark datasets.}
	\label{tab:datasetSpec}
	\begin{tabular}{|c|c|c|}
	\hline
	Dataset 		& \# of reactions	& \# of non-zero variables ($p$)  \\
	\hline
	iML1515 			& 2712 							& 2326						\\
	\hline
	iEC1372\_W3110 			& 2758 						& 2339						\\
	\hline		
	iECDH10B\_1368 		& 2742 							& 2252						\\
	\hline
	iY75\_1357 & 2759 							& 2249						\\
	\hline
	iAF1260b 		& 2388 							& 1588					   \\
	\hline
	iAF1260 	& 2382 							& 1633						\\
	\hline
	iJR904 & 1075 							& 770						\\
	\hline
	E.coli Core &
	95								&	 85 \\
	\hline
	\end{tabular}
\end{table} 

We utilize seven Genome-scale metabolic networks as our benchmarks \cite{feist2007genome, reed2003expanded, monk2017ml1515, orth2011comprehensive, monk2016multi, monk2013genome, feist2010model} to evaluate the performance of ParaLiNGAM.
The metabolites are molecules involved in chemical reactions in a cell, and sets of these chemical reactions are so-called Metabolic networks \cite{lacroix2008introduction}. 
These metabolic networks can be studied in silico with  flux balance analysis \cite{orth2010flux} which is a way to simulate metabolic networks and to measure effects on the system by external
influences. The flux balance analysis is utilized to generate datasets.
The data generation procedure is performed with COBRA-toolbox \cite{becker2007quantitative, schellenberger2011quantitative}, and it considers the metabolic network of the Escherichia coli bacteria str. K-12. In order to utilize these networks, we acquire their models from BiGG Models\cite{king2016bigg}.

To generate data, first, we import models from BiGG models in COBRA. Then, utilizing COBRA's optGpSampler \cite{megchelenbrink2014optgpsampler}, we generate data by uniformly sampling from solution space with hit and run algorithm.
In this algorithm, first, $n$ points (samples) are generated in the middle of the solution, and then these points are relocated in a random direction. Although, after substantial steps in this procedure, some reactions' samples remain zero. These reactions are removed from datasets.

Details of the generated datasets are shown in Table ~\ref{tab:datasetSpec}. The first column shows the number of reactions, and the second column shows the number of non-zero variables among these reactions.
Each variable (reaction) is generated with $10000$ samples.

\subsection{Performance Comparison}

\subsubsection*{Comparing ParaLiNGAM with DirectLiNGAM }

The runtimes of both DirectLiNGAM and ParaLiNGAM are reported in Table \ref{tab:realTimings}.  The accuracy of the proposed solution is exactly the same as the DirectLiNGAM. Thus, we only report runtime of these experiments.
The third column shows serial runtime. The serial runtime on iJR904 dataset is 287780 seconds (approximately 3.3 days). 
Since the computational complexity has cubic relation with respect to the number of variables, the runtime of iAF1260b dataset, which is the next smallest dataset after iJR094, would probably be longer than three weeks. Thus, it is impractical to measure the runtime for other datasets, and the serial runtime is reported just for two datasets, which is 485 seconds for E.coli Core and 287780 seconds for iJR904. More comparisons with the serial solution is reported in Section \ref{sec:scalability} for synthetic datasets.

The fourth column reports runtime of ParaLiNGAM for all datasets, which ranges from 759 milliseconds to 91.3 seconds. The speedup ratio over serial execution for measured datasets is up to 3152.


\begin{table*}[tp]
	\centering
	\caption{Comparing the serial and parallel implementations. The third and fourth columns show the runtimes. The last column shows the speedup ratio, which is calculated by dividing the serial runtime over the parallel runtime.}
	\label{tab:realTimings}
	\begin{tabular}{|c|c|c|c|c|c|}
	\hline
	Dataset 		& \# of variables	& Serial runtime (sec.)  & GPU runtime (sec.) & Speedup ratio \\
	\hline
	iML1515 		& 2326	 & \textemdash \textemdash	& 1321			 & \textemdash \textemdash\\
	\hline
	iEC1372\_W3110	& 2339	 & \textemdash \textemdash	& 1420			& \textemdash \textemdash \\
	\hline		
	iECDH10B\_1368 	& 2252	&  \textemdash \textemdash & 1216			& \textemdash \textemdash \\
	\hline
	iY75\_1357 		& 2249	&  \textemdash \textemdash & 1174			& \textemdash \textemdash \\
	\hline
	iAF1260b 		& 1588	&  \textemdash \textemdash & 507			& \textemdash \textemdash \\
	\hline
	iAF1260 		& 1633	&  \textemdash \textemdash & 518			& \textemdash \textemdash \\
	\hline
	iJR904 			& 770	& 287780 ($\sim$3.3 days)	& 91.3	& 3152			\\
	\hline
	E.coli core 	& 85	& 485		& 0.759	& 638\\
	\hline
	
	\end{tabular}
\end{table*}
\subsubsection*{Comparing ParaLiNGAM with Other Parallel Methods}

Herein, three baseline parallel algorithms are introduced, and their performance are compared against the proposed ParaLiNGAM algorithm. See Fig. \ref{fig:baseLineTiming}. The first baseline algorithm is formed by assigning each variable to a block, and blocks compare themselves to each other. In specific, we have blocks equal to the number of remaining variables in each iteration, and each block performs one comparison at a time. We call this algorithm \textbf{Block Worker}.

The second baseline algorithm is similar to the previous one, in that  each variable is assigned to a block, but in each block, threads are responsible for different comparisons. Hence, each block can perform comparisons simultaneously. Since running lots of comparisons in parallel requires a lot of memory, this method cannot fit in GPU for large numbers of variables. In specific, we need separate memory for normalized variables and calculated residuals (see Compare Function in Algorithm \ref{alg:baseLiNGAM_FR}). As a result, we need $O(r^2 n)$ memory ($r$ is the number of remaining variables) in each iteration, which is problematic for large datasets. However, in Block Worker, we have just $r$ simultaneous comparison at a time and require just $O(r n)$ memory, which is a moderate value. 
%
Hence, we need to optimize memory usage in this algorithm. 
In specific, we store parameters like mean, variance, and covariance of comparing variables used in calculations. Then, we merely read input data from memory to perform comparisons. This solution not only solves memory issues but also reduces the runtime by avoiding redundant memory reads and writes. We call this algorithm \textbf{Thread Worker}.


In the third baseline algorithm, in each iteration, every comparison is assigned to a block, i.e., we have $r\times r$ blocks ($r$ is the number of remaining variables), and block of index $(i, j)$ compares $X_i$ with $X_j$. Like the previous baseline algorithm, performing many comparisons in parallel requires a lot of memory. Therefore, the above  mentioned optimizations are utilized to reduce memory usage in this algorithm as well. We call this algorithm \textbf{Block Compare}.

%In all of these baseline algorithms, all computational optimizations for pre-processing and post-processing of data are utilized same as ParaLiNGAM. Furthermore, different configurations were tested, and the best of them is reported. \blue{rewrite this paragraph}


%\begin{figure*}[tp]
%\centering
%\includegraphics[width = \linewidth]{fig/baseLine}
%\caption{Comparing the performance of  ParaLiNGAM with three baseline GPU-parallel algorithms. Every bar illustrates a ratio between two time values.}
%\label{fig:baseLineTiming}	
%\end{figure*}

\begin{figure*}[tp]
\centering
\includegraphics[width = \linewidth]{fig/baseLine}
\vskip -3mm
\caption{Comparing the performance of  ParaLiNGAM with three baseline algorithms on GPU. Every bar illustrates speedup ratio between the base line algorithm and ParaLiNGAM.}
\label{fig:baseLineTiming}	
\end{figure*}


As illustrated in Fig. \ref{fig:baseLineTiming}, ParaLiNGAM  is 16 X to 2.4 X faster than the Block Worker method, 11.5 X to 6.7 X faster than Thread Worker, and 10.4 X to 1.1 X faster than Block Compare. Note that E.coli Core dataset has fewer variables compared to other datasets, and it under-utilizes the GPU. 
%
In most cases, Block Worker has the worst performance among the three baseline methods. This is due to its inefficient memory usage. Between Thread Worker and Block Compare, the first method employs too much parallelism, and threads of each block try to access  different parts of memory, which is less efficient compared with Block Compare, in which, there is a limited number of concurrent comparisons (number of blocks that can run simultaneously on the GPU). 
%
%Moreover, different speedups among datasets are due to threshold mechanism which will be discussed in Section \ref{sec:exp:config}

%\subsection{Impact of the Threshold Mechanism}
%\label{sec:exp:config}
%
%The threshold mechanism that was proposed in Section \ref{sec:thresh}  has a significant impact on reducing the number of comparisons in iterations. 
%%
%Table \ref{tab:updateRate} shows the number of comparisons saved for different values of $c$ (update rate). As we increase the value of $c$, more comparisons are performed in each step of iterations, so the total percentage of saved comparisons decreases. On the right side of the table, runtimes of these experiments are shown. As detailed in the table, saving more comparisons does not necessarily lead to smaller runtime. Because in ParaLiNGAM (Algorithm \ref{alg:SchedulerV2}), we re-launch the GPU kernel after each threshold update. Hence, updating the threshold value many times can cause too much delay, which is not efficient. The minimum runtime for each dataset is colored green. As the number of variables increase, smaller values for $c$ can be more beneficial due to more number of saved comparisons.
%As shown in the table, $c=2$ gives the best runtime for experimented datasets with more than 2000 variables. However, for smaller datasets, $c=5$ yields better runtime. Moreover, for a much smaller dataset E. coli core, $c=10$ or a higher value can be more suitable.

%
%\red{I think it is better to delete it. It is not a good place to give a new idea!}
%\blue{we can delete this second strategy part...}
%It is noteworthy to mention that there is an alternative strategy to deploy a threshold mechanism for smaller datasets. In the default strategy, threshold value resets in every iteration, which maximizes saved comparisons, but leads to more kernel launches. The alternative strategy is defining a global threshold for the whole execution, and after each update, the threshold value keeps its updated value for the rest of the execution.
%The latter strategy leads to fewer kernel updates but cannot save comparisons as much as the previous strategy.
%
%%Although, this is not a major issue, because both strategies have similar performance in the first iterations.
%%In the last iterations, the second strategy has a higher threshold value than the first strategy, but there are not many comparisons left in execution, hence the total number of comparisons saved has no major difference in the two strategies.
%
%Choosing an efficient strategy for the threshold mechanism depends on the time is spent on comparisons and kernel launch.
%If comparing two variables is a time-consuming task on deployed hardware or there are a lot of comparisons, the first strategy is more beneficial by saving more comparisons. On the other hand, the second strategy can be more efficient if comparing variables does not take much time, and the number of kernels we launch has a considerable proportion of total runtime.

%\begin{table*}[tp]
%\centering
%\caption{Percentage of saved comparisons and runtime of ParaLiNGAM for different values of $c$. Green color indicates the minimum runtime in each dataset.
%%\blue{shall we add number of variables?} \red{NO!}
%}
%\label{tab:updateRate}
%\begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|}
%\hline
%%\multicolumn{2}{|c|}{}
%	
%	\multicolumn{1}{|c|}{} & \multicolumn{5}{c||}{Percentage of saved comparisons} & \multicolumn{5}{c|}{GPU Runtime (sec.)}\\
%	\hline
%	\rowcolor{orange!50}$c$ &  1.05	& 1.5	& 2	&5 &10	& 1.05	& 1.5	& 2	&5 &10 \\
%	\hline
%	iML1515 	& 92 &	90.8 & 89.6 & 86.8 & 84.1 & 1829	& 1345	& \cellcolor{green!50}1321	& 1335	& 1384 \\
%	\hline
%	iEC1372\_W3110 		& 92.4 & 91.4 & 90.8	& 85.7	& 83
%	& 2052	& 1477	& \cellcolor{green!50}1420	& 1509	& 1552 \\
%	\hline		
%	iECDH10B\_1368 		& 92.5	& 91.4	& 90.8	& 86.4	& 82.1
%	 & 1766	& 1237	& \cellcolor{green!50} 1216	& 1257	& 1342
%	 \\
%	\hline
%	iY75\_1357 			& 93.1	& 91.9	& 91.1	& 87	& 83.2 & 1639	& 1201	& \cellcolor{green!50} 1174	& 1229	& 1305 \\
%	\hline
%	iAF1260b 			& 90.7	& 89.3	& 88.3	& 85	& 82.1
%	 & 821	& 532	& 507	& \cellcolor{green!50} 495	& 506 \\
%	\hline
%	iAF1260 			& 93	& 92.1	& 91.3	& 88.1	& 85.4
%	 & 858	& 549	& 518	& \cellcolor{green!50} 510	& 520
%	 	\\
%	\hline
%	iJR904 				& 90.8	& 89.9	& 89.2	& 85.9	& 84.3
%	 &172	& 100.4	& 91.3	& \cellcolor{green!50} 84.2	& 81.3 \\
%	\hline
%	E.coli Core 		& 82.5	& 81.8	& 81	& 77.6	& 74.1
%	 & 1.60	& 1.12	& 0.759	& 0.731	& \cellcolor{green!50} 0.695 \\
%	\hline
%\end{tabular}
%\end{table*}


\subsection{Scalability}
\label{sec:scalability}
In this section, we evaluate the scalability of ParaLiNGAM. In particular, we measure the runtime of our proposed algorithm against DirectLiNGAM for different numbers of variables ($p$) and samples ($n$). %\red{Speedup ratio increases as the size of the dataset grows.}
 
We follow a similar procedure as ICA-LiNGAM \cite{shimizu2006linear} for the data generation mechanism.
First, we choose the number of parents for each variable, and generate a random matrix for adjacency matrix $B$. In sparse graphs, the number of parents is uniformly selected from interval $[1, 0.2 p]$, and for dense graphs the interval is $[0.25 p, 0.5p]$ ($p$ is number of variables).
Next, non-zero entries of $B$ are replaced with a random value, from interval $[-0.5, -0.95] \bigcup [0.5, 0.95]$.
Next, we generate exogenous noise $N_i$ for each variable by sampling from Gaussian distribution, then pass them through a power non-linearity (keeping same sign, but changing the absolute value to an exponent in interval $[0.5, 0.8] \bigcup [1.2, 2]$).
Finally, we generate samples for all variables recursively and permute them randomly. For this section, datasets are generated for number of variables of $p = 100, 200, 500, 1000$ and sample sizes of $n = 1024, 2048, 4096, 8192$.

%\red{Please do not use '-' in dataset!}

% Furthermore, in ParaLiNGAM, most mechanisms have same performance regardless of graph density, except the threshold mechanism.

%Since, the density of graphs is not important for DirectLiNGAM, and for some datasets, it takes more than several days to execute, a random dataset is considered as benchmark.

As mentioned earlier, the proposed solution does not change the algorithm accuracy and has the same precision. Therefore, only the runtime of the algorithms are shown in Fig. \ref{fig:syntheticTiming} for sparse and dense graphs.

\begin{figure*}[tp]
\centering
\includegraphics[width = 1.05 \linewidth]{fig/synTime}
\caption{Runtimes of ParaLiNGAM  and DirectLiNGAM for  a) sparse graphs and b) dense graphs for different number of variables and sample sizes.}
\label{fig:syntheticTiming}	
\end{figure*} 

In Fig. \ref{fig:syntheticTiming}, each column shows runtime for $p=100, 200, 500, 1000$, and rows (a) and (b) show runtime for sparse and dense graphs, respectively. The runtimes of sparse graphs are similar to dense graphs for DirectLiNGAM algorithm, due to the same procedure and computations. In particular,  the independent test is performed for all pairs of variables in all iterations despite the graph density. Hence, runtime merely depends on the number of variables and samples. The runtime of DirectLiNGAM varies from 71.4 seconds to 658806 seconds ($\sim$ 7.6 days). However, ParaLiNGAM attains a much smaller runtime compared with DirectLiNGAM, and its runtime varies from 119 milliseconds to 151 seconds. The speedup ratio of the proposed algorithm over the serial implementation ranges from 536 X to 4657 X. Furthermore, the speedup ratio increases as $p$ and $n$ increase.

%Each of Tables \ref{tab:synGraphs} and \ref{tab:synGraphsDense}, consists four sub-tables for $p=100, 200, 500, 1000$. In each subtable, the runtime of serial and GPU, and speedup ratio of GPU  against serial is reported. Serial runtime varies from 104 seconds to 852480 seconds ($\sim$ 10 days), and it increases as the size of graph grows. However, ParaLiNGAM attains a much smaller runtime compare to serial implementation. The proposed solution's runtime varies from 110 milliseconds to 146 seconds. The speedup ratio of the proposed algorithm over the serial implementation ranges from 945 X to 6325 X. Moreover, speedup ratio increases as $p$ and $n$ increase.





%\begin{table*}[tp]
%	\centering
%	\caption{Runtime of ParaLiNGAM  and DirectLiNGAM for sparse graphs in different number of variables and sample sizes.}
%	\label{tab:synGraphs}
%		
%	\begin{tabular}{|c|c|c|c|}
%%		\caption{$p= 100$}
%		\hline
%		\# of samples($n$)		& Serial (sec.)	&  GPU (sec.) & Speedup \\
%		\hline
%		1024	& 104	& 0.11 & 945.45 \\
%		\hline
%		2048	& 214	& 0.15 & 1426.67 \\
%		\hline
%		4096	& 438	& 0.25 & 1752 \\
%		\hline
%		8192	& 886	& 0.425 &  2084.71 \\
%		\hline
%	\end{tabular}
%	\hfil
%	\begin{tabular}{|c|c|c|c|}
%%		\caption{$p= 200$}
%		\hline
%		\# of samples($n$)		& Serial (sec.)	& GPU (sec.) & Speedup \\
%		\hline
%		1024	& 852	& 0.45 &  1893.33 \\
%		\hline
%		2048	& 1714	& 0.65 &  2636.6 \\
%		\hline
%		4096	& 3502	& 1.06 &  3303.77 \\
%		\hline
%		8192	& 7089	& 1.8 &  3938.33 \\
%		\hline
%	\end{tabular}
%	\\
%	\medskip
%	\hfill$p = 100 $ \hfill  \hfill $p = 200$ \hfill
%	\bigskip
%		
%	\begin{tabular}{|c|c|c|c|}
%%		\caption{$p= 500$}
%		\hline
%		\# of samples($n$)		& Serial (sec.)	& GPU (sec.) & Speedup \\
%		\hline
%		1024	& 13295	& 4.3 & 3091.86 \\
%		\hline
%		2048	& 26712	& 6.4 & 4173.75 \\
%		\hline
%		4096	& 54720	& 10 & 5472 \\
%		\hline
%		8192	& 110688 & 17.5 &  6325.03 \\
%		\hline
%	\end{tabular}	
%	\hfil
%	\begin{tabular}{|c|c|c|c|}
%%		\caption{$p= 1000$}
%		\hline
%		\# of samples($n$)		& Serial (sec.)	& GPU (sec.) & Speedup \\
%		\hline
%		1024	& 106559	& 35.5 & 3001.66  \\
%		\hline
%		2048	& 213120	& 47.5 & 4486.7  \\
%		\hline
%		4096	& 426239	& 77.5 & 5499.86  \\
%		\hline
%		8192	& 852480	& 146 & 5838.9  \\
%		\hline
%	\end{tabular}
%	\\
%	\medskip
%	\hfill$p = 500 $ \hfill  \hfill $p = 1000$ \hfill
%	\medskip
%\end{table*} 
%
%\begin{table*}[tp]
%	\centering
%	\caption{Runtime of ParaLiNGAM  and DirectLiNGAM for dense graphs in different number of variables and sample sizes. \blue{to be completed}}
%	\label{tab:synGraphsDense}
%		
%	\begin{tabular}{|c|c|c|c|}
%%		\caption{$p= 100$}
%		\hline
%		\# of samples($n$)		& Serial (sec.)	&  GPU (sec.) & Speedup \\
%		\hline
%		1024	& 104	& 0.11 & 945.45 \\
%		\hline
%		2048	& 214	& 0.15 & 1426.67 \\
%		\hline
%		4096	& 438	& 0.25 & 1752 \\
%		\hline
%		8192	& 886	& 0.425 &  2084.71 \\
%		\hline
%	\end{tabular}
%	\hfil
%	\begin{tabular}{|c|c|c|c|}
%%		\caption{$p= 200$}
%		\hline
%		\# of samples($n$)		& Serial (sec.)	& GPU (sec.) & Speedup \\
%		\hline
%		1024	& 852	& 0.45 &  1893.33 \\
%		\hline
%		2048	& 1714	& 0.65 &  2636.6 \\
%		\hline
%		4096	& 3502	& 1.06 &  3303.77 \\
%		\hline
%		8192	& 7089	& 1.8 &  3938.33 \\
%		\hline
%	\end{tabular}
%	\\
%	\medskip
%	\hfill$p = 100 $ \hfill  \hfill $p = 200$ \hfill
%	\bigskip
%		
%	\begin{tabular}{|c|c|c|c|}
%%		\caption{$p= 500$}
%		\hline
%		\# of samples($n$)		& Serial (sec.)	& GPU (sec.) & Speedup \\
%		\hline
%		1024	& 13295	& 4.3 & 3091.86 \\
%		\hline
%		2048	& 26712	& 6.4 & 4173.75 \\
%		\hline
%		4096	& 54720	& 10 & 5472 \\
%		\hline
%		8192	& 110688 & 17.5 &  6325.03 \\
%		\hline
%	\end{tabular}	
%	\hfil
%	\begin{tabular}{|c|c|c|c|}
%%		\caption{$p= 1000$}
%		\hline
%		\# of samples($n$)		& Serial (sec.)	& GPU (sec.) & Speedup \\
%		\hline
%		1024	& 106559	& 35.5 & 3001.66  \\
%		\hline
%		2048	& 213120	& 47.5 & 4486.7  \\
%		\hline
%		4096	& 426239	& 77.5 & 5499.86  \\
%		\hline
%		8192	& 852480	& 146 & 5838.9  \\
%		\hline
%	\end{tabular}
%	\\
%	\medskip
%	\hfill$p = 500 $ \hfill  \hfill $p = 1000$ \hfill
%	\medskip
%\end{table*} 



%\begin{figure*}[tp]
%\centering
%\includegraphics[width = \linewidth]{fig/synTime}
%\caption{Runtime of ParaLiNGAM  and DirectLiNGAM for dense graph in different number of variables and sample sizes. \blue{to be completed}}
%\label{fig:syntheticTimingDense}	
%\end{figure*}



==> LiNGAM(A23) - arXiv/imp.tex <==
\section{Implementation Details}
\label{sec:alg2}

Further details on the proposed parallel algorithm is presented in this section. First, a short background on CUDA is presented in Section \ref{sec:CUDA}. Further details on our GPU implementation are discussed in Sections \ref{sec:GPUImp} and \ref{sec:schGPU}.

%\subsection{Balancing Comparisons}
%\label{sec:workBalance}
%
%\begin{figure}[tp]
%	\centering
%	\includegraphics[width =  \columnwidth]{fig/CompareBalance2}	
%	\caption{Illustration of balancing comparisons. On the left side, $\mathcal{C}$ is initialized with $1$, and workers compare themselves with the first worker at the beginning of iterations. On the right side, $\mathcal{C}[w] = w+1$, and workers compare themselves with their following worker.
%	Gray color indicates already performed comparisons, green color shows the comparisons performed in the step, and blue color represents the comparisons performed by messaging mechanism.
%%	\blue{Another version with five variables is available in fig/CompareBalance.}
%	}
%	\label{fig:alg:balance} 
%\end{figure}
%
%We discuss the advantages of the scheduling method through an example. Please see Fig. \ref{fig:alg:balance}. Suppose we have seven workers in an iteration which can perform their computations simultaneously. 
%As mentioned in Algorithm \ref{sec:scheduler}, workers start their comparisons from the first worker. Hence, 
%in the first step of iteration (and other iterations), all comparisons of worker $1$'s are performed by itself or other workers (and informed with messaging mechanism). As a result, after the first step, worker $1$ finishes its task, and its final score in the iteration is computed.
%A similar situation happens for the worker $2$ in the second step and so on. However, this procedure has some drawbacks.
%First, after two steps of the illustrated example, workers $6$ and $7$ have performed just two comparisons by themselves, and messaging mechanism has not helped them yet. Second, after each step, a worker is terminated, which is inefficient and causes iterations to take more steps to finish. Finally, the threshold mechanism cannot perform efficiently. As mentioned in Section \ref{sec:thresh}, threshold mechanism controls number of active workers by gradual progress of their scores. However, in the mentioned procedure, this mechanism does not perform properly for workers like $1$ and $2$ that have finished their tasks early. Furthermore, score updates for some workers (like $6$ and $7$ in this example) are too slow, and it is more efficient to update such workers' scores more often.
%
%A solution to this problem is by initializing $\mathcal{C}$ in a different manner for each worker (please see the right figure in Fig. \ref{fig:alg:balance} for an example of this initialization). In this example, workers start comparing themselves with their following workers ($\mathcal{C}[w] = w+1$). Next, we increase each value (in a wrap-around manner) until it reaches to $w$.
%Hence, in each step, each worker performs a comparison and is informed about another comparison. This way of initialization can balance the comparisons for all workers, and the threshold mechanism will be more beneficial. Moreover, it has not problems mentioned earlier in this section, and all workers can be present till the end of an iteration, and iterations take fewer steps. 

\subsection{CUDA}
\label{sec:CUDA}

% from cuPC paper
CUDA is a parallel programming API for Nvidia GPUs. GPU is a massively parallel processor with hundreds to thousands of cores.
%
CUDA follows a hierarchical programming model. At the top level, computationally intensive functions are specified by the programmer as CUDA \textbf{kernels}. For briefness, from now on, we use kernel instead of CUDA kernel. A kernel is specified as a sequential function for a single \textbf{thread}. The kernel is then launched for parallel execution on the GPU by specifying the number of concurrent threads. 

Threads are grouped into \textbf{blocks}. A GPU kernel consists of a number of blocks, and every block consists of a number of threads.
%
%Every block has access to a small, on-chip, and low-latency memory, called \textbf{shared memory}. The shared memory of a block is accessible to all threads within that block, but not to any thread from other blocks.

In order to identify blocks within a kernel, and threads within a block, a set of indices are used in the CUDA API, for instance, $blockIdx.x$ denotes  the block index in dimension $x$ within a kernel. 

%There are other dimensions for blocks and also for threads, but we just use blocks in the proposed algorithms {\color{red} What do you mean here?}. However, threads are used in function implementations to help them run faster by dividing tasks and samples between them. 


%and $threadIdx.x$ as the thread index in dimension $x$ within a block. There are other dimensions in CUDA, but for brevity, we only use them and denote these two indices as $bx$ and $tx$, respectively.

\subsection{GPU Implementation}
\label{sec:GPUImp}
%So far, we have discussed some aspects of ParaLiNGAM.
In this section, we present further details on the implementation of ParaLiNGAM on GPU hardware. 
In the ParaLiNGAM algorithm, we used workers to handle variables' tasks. In CUDA, we assign workers to blocks. Moreover, each block can divide its computations among parallel threads to improve the performance, e.g., for performing tasks like $CheckMessages$ and $Compare$. Herein, for brevity of notation, we denote $blockIdx.x$ by $w$.
Now we discuss two approaches to implement ParaLiNGAM on GPU.

The first approach is to assign fewer threads to each block and decrease the computation power of each block, in the meantime, run all of the blocks together. 
Thereby, a whole iteration can be launched by one kernel. Moreover, we can perform scheduling in GPU by considering one block for the scheduler, i.e., all blocks but one skip scheduling part based on their block IDs.

However, this solution has some drawbacks.
First, each worker requires its own exclusive memory. Hence, all workers may not fit in GPU memory. As a result, it is not scalable, and we cannot utilize it for large number of variables.
%Second, it needs synchronization within the kernel to control blocks on each step and reschedule them.
%%As mentioned earlier, threads are grouped as a block, and threads can be synchronized in one block due to hardware facilities \red{limitations?}.
%But, synchronizing all threads in the kernel is time-consuming due to using atomic operations or barrier synchronization (\red{needs some citation}).
%\blue{I did not mention grid synchronization here, and we can discuss it in the next meeting.} \red{Ok!}
Moreover, blocks are slower due to the smaller number of threads. As a result, this approach would be time-consuming, even if all the blocks fit in the GPU.

The second approach is to run $Compare$ and $CheckMessages$ tasks in separate kernels on GPU while performing the scheduling task on the host (CPU). This approach is scalable and does not have the above problems. However, launching kernels is time-consuming. Moreover, we launch two kernels separately for each step, which is not efficient.
Unlike the first approach, we can consider some modifications to the second approach in order to improve its performance, which is discussed in the next part.


\subsection{Scheduling on GPU}
\label{sec:schGPU}

In order to resolve second approach's issues, one solution is to relax the synchronization between $Compare$ and $CheckMessages$. In Algorithm \ref{alg:ParaLiNGAM_FR}, we consider a barrier between these two functions (lines $9$ and $10$) in order to update the score of workers faster by checking their messages only after all messages are received. 
%
However, removing the barrier causes some workers to receive their messages later in the further steps. Hence, relaxing the synchronization causes a delay in delivery of some messages, however, it halves the kernel launching delays, which is quite beneficial. As a result, the workers (blocks) can compare and check for messages independently, and thus, we can merge $Compare$ and $CheckMessages$ kernels. Still, assigning each step to a kernel and evaluating iteration status by the host is not an efficient option and causes too many kernel calls. Therefore, the procedure of scheduling must be revised.

In ParaLiNGAM, a worker can perform just one comparison (if it is active) in each step. This limitation was due to the synchronization of $Compare$ and $CheckMessages$, which is now relaxed. 
Hence, now we can divide an iteration into steps by threshold updates, instead of performing one comparison per worker. In other words, workers now can continue their comparisons to reach the threshold instead of just performing one comparison. 
%
To implement this solution, we modify some of the scheduler's tasks in order to move them to the worker.  Scheduler has three tasks: checking termination of an iteration, updating the threshold, and updating $\mathcal{C}$. Now, we discuss modifications that are needed in these three tasks.

In the first task, i.e., checking iteration's termination, worker $w$ can keep track of its finished comparisons by checking $\mathcal{D}[w]$. 
Therefore, workers can continue to compare themselves with each other till they reach the threshold or finish their comparisons. Moreover, they can announce their state by $finish$ flag.

The second task is updating the threshold, which is a mechanism to divide iteration into steps.
In Algorithm \ref{alg:ParaLiNGAM_FR}, workers synchronize before updating the threshold.
As mentioned before, synchronizing a kernel is not efficient. Hence, we update the threshold outside of the kernel in the host.
In Section \ref{sec:scheduler}, constant $c$ is introduced to control the amount of change in threshold in each update. 
In particular, higher values for $c$ would cause increasing the number of comparisons. However, it can be more efficient due to fewer kernel calls. As a result, this parameter must be adjusted according to the number of tests, test duration, and launching kernel delays.

In the last task, workers can also determine their comparisons' target by checking their unfinished workers in $\mathcal{D}$.

Now we discuss changes in the main algorithms to implement them on GPU which are given in Algorithm \ref{alg:SchedulerV2} and Algorithm \ref{alg:GPUKernel}.

Main loop of Algorithm \ref{alg:ParaLiNGAM_FR}  (lines $14-18$) is replaced to Algorithm \ref{alg:SchedulerV2}. In this algorithm, $\mathcal{C}$ is modified for more efficiency, and also functions of $Compare$, $CheckMessages$ and some parts of $Scheduler$ are moved to $GPUKernel$ (Algorithm \ref{alg:GPUKernel}).


\begin{algorithm}%[tp]
	\begin{algorithmic}%[1]
		\State $\mathcal{C} = [2, 3, ..., r, 1]$
		\State $finish = False$
		\Repeat
			\State GPU: $finish, State = GPUKernel(\mathcal{W},
			State)$
			\State $\gamma *= c$
		\Until{$finish$}
		
	\end{algorithmic}
	\caption{$ParaLiNGAM~Code patch$} 
	\label{alg:SchedulerV2}
\end{algorithm}

The description of $GPUKernel$ is given in Algorithm \ref{alg:GPUKernel}.
The main part of the algorithm is a loop in lines $1-13$. A worker's task is completed if it compares itself to all other workers, which is checked in line $13$.

In line $2$, same as line $14$ of Algorithm \ref{alg:ParaLiNGAM_FR}, workers check for their messages. Since GPU has limited resources, it makes a queue for blocks if it cannot fit them on its streaming multiprocessors (SMs). Hence, some workers launch later, therefore, checking messages as the first task would help them gain information from other previously active workers and check their scores to see if they have already reached the threshold.

In lines $3-5$, workers check their scores to see if they reached the threshold. In that case, they have to stop for this step and wait for the threshold update.
Then, in lines $6-8$, workers also check for termination of the iteration, and if they have finished their comparisons after checking messages, they set $finish$ as $True$.

Next, in lines $9-11$, workers choose their comparison target by increasing $\mathcal{C}[w]$.
Then, workers perform their comparisons in line $12$. Finally, if a worker finishes comparisons without reaching the threshold, it sets $finish$ as $True$ and notifies the host scheduler that  is the end of the current iteration.

In line $22$ in Algorithm \ref{alg:Scheduler}, we used a condition to avoid redundant comparisons. In discussed implementation on GPU, we perform comparisons asynchronously. Hence, checking redundant comparisons is not straightforward as before, and we need to use more complicated mechanisms. For brevity, such details are not mentioned in the algorithms. But, in short, for this matter, we utilize a flag for each comparison, and workers try to lock them with atomicCAS operation.
Moreover, if a worker reaches some comparison that its flag is already set, the worker skips that comparison and would receive that comparison's result later.

\begin{algorithm}[h]
	\begin{algorithmic}[1]
		\Input $State$
		\Output $finish$
		\Block p
%		\Thread $N_{th}$
		\Repeat
			\State $\mathcal{S}[w] += CheckMessages(w, State)$\hfill //Check
			\If {$\mathcal{S}[w] > \gamma$}\hfill //Evaluate
				\State \textbf{Exit}
			\EndIf
			\If {$\mathcal{D}[w, :]$ is all $True$}
				\State \textbf{break}
			\EndIf
			\Repeat \hfill // Compare
				\State $\mathcal{C}[w] = (\mathcal{C}[w]+1)\%size(U)$
			\Until{$\mathcal{D}[w][\mathcal{C}[w]]$ is $False$}
			\State $\mathcal{S}[w] += Compare(w, \mathcal{C}[w], state)
			\hfill$
%Section \ref{sec:compare}
		\Until{$\mathcal{D}[w, :]$ is all $True$}
		\State $finish = True$
	\end{algorithmic}
	\caption{$GPU Kernel$} 
	\label{alg:GPUKernel}
\end{algorithm}

%\begin{figure}[tp]
%	\centering
%	\includegraphics[width = 0.9 \columnwidth]{fig/Part32}	
%	\caption{Illustration of ParaLiNGAM execution for first iteration of Example \ref{ex:pre}, which is performed in one step.} 
%	\label{fig:alg:ex} 
%\end{figure}
%
%\begin{Example}
%Fig. \ref{fig:alg:ex} illustrates the procedure of parallel execution for Example \ref{ex:pre}. Suppose GPU has capacity for only two workers (blocks) to work simultaneously and others stay in a queue. Moreover, for simplicity of illustration, active workers simultaneously perform the same phase (i.e., Check, Evaluation, Compare). Also, the threshold is equal to $0.05$.
%
%First, workers $1$ and $2$ start their tasks. They check for their messages, which are empty. Next, they determine their target workers to compare themselves. Next, they perform their comparisons, update their scores, and send messages to compared workers. Next, in the check phase, worker $1$ does not have any message, but worker $2$ has a new message from worker $1$ and updates its score. In the evaluation phase, worker $2$ terminates because it has reached the threshold.
%
%Now, worker $3$ can start its comparisons. First, it checks for messages and marks worker $2$ as "done". Worker $3$'s score is below than the threshold. Therefore, it continues the compare phase. Workers $1$ and $3$ compare themselves to $3$ and $4$ and send messages accordingly. They check for their messages in the check phase. In the evaluation phase, worker $1$ terminates due to its score.
%
%Now, worker $4$ starts its task and checks for messages from other workers. It receives a message from worker $3$ and terminates afterward without performing any comparisons because its score is higher than the threshold.
%
%Finally, worker $5$ starts its task. It goes to compare phase because it has no messages. Worker $3$ and $5$ start compare phase, and they send messages to compared workers. Worker $5$ terminates because of its score. On the other hand, worker $3$ has finished its comparisons. At this point, GPU Kernel's task is completed. All workers either terminated or finished their comparisons. At last, the host chooses worker $3$'s variable as the root.
%
%In this example, for simplicity, iteration is finished within one step, and we did not update the threshold. However, in practice, the root's score may not be exactly zero, and an iteration takes place in multiple steps.
%
%\end{Example}


%\section{Extra}
%\label{sec:extra}
%
%%we have to use thread fence.
%
%renaming is done for better memory access.
%
%Lock mechanism
%
%%for lock we use some memory and use atomicCAS to keep it lock for an operation
%%%
%
%\subsection{Compare}
%\label{sec:compare}
%There is better implementation with reusing variable which is not discussed for brevity(!).
%
%reusing variables
%\begin{algorithm}[tp]
%	\begin{algorithmic}[1]
%		\Input $x_{dim}, x_j, \Sigma$
%		%\Output 
%		\State $Lock(dim , j)$
%		\State $r_j^{dim} =\dfrac{1}{\sqrt{1 - \Sigma[dim][j]^2}} (x_{dim} - \Sigma[dim][j] x_j)$
%		\State $\mathcal{E}[dim][j] = Entropy(r_j^{dim})$
%		\State $r_{dim}^j =\dfrac{1}{\sqrt{1 - \Sigma[j][dim]^2}} (x_j - \Sigma[j][dim] x_{dim})$
%		\State $\mathcal{E}[dim][j] = Entropy(r_j^{dim})$
%		\State $Lock(j , j)$
%		\State $\mathcal{E}[j][j] = Entropy(x_j)$
%		\State $result = \mathcal{E}[j][j] + \mathcal{E}[dim][j] - (\mathcal{E}[dim][dim] + \mathcal{E}[j][dim])$
%		\If {$result < 0$}
%			\State $Scores[dim] += result^2$
%		\EndIf
%		\State $SendMessage(j, result)$
%	\end{algorithmic}
%	\caption{Compare function}
%	\label{alg:Compare}
%\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> LiNGAM(A23) - arXiv/intro.tex <==
\section{Introduction}
\label{sec:intro}

% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.
%\IEEEPARstart{T}{his} 
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)
%I wish you the best of success.
%
%\hfill mds
% 
%\hfill August 26, 2015
\IEEEPARstart{D}{iscovering} the underlying causal mechanism in various natural phenomena or human social behavior is one of the primary goals in artificial intelligence and machine learning. For instance, we may be interested in recovering causal relationships between different regions of brain by processing fMRI signals \cite{huang2021diagnosis,sanchez2019estimating} or estimating causal strengths between genes in a gene regulatory networks (GRN) by observing gene expression levels \cite{marbach2012wisdom,haury2012tigress}. Having access to such causal relationships can enable us to answer to interventional or counter-factual questions which has broad impacts on designing a truly intelligent system \cite{pearl2018book}. The golden standard for the causal discovery is through conducting controlled experiments. Unfortunately, performing experiments in a system might be too costly or even infeasible \cite{ghassami2018budgeted}. As a result, there have been extensive studies in the literature of causality to recover causal relationships from merely observational data \cite{peters2017elements}.

Causal relationships among a set of variables can be represented by a directed acyclic graph (DAG) where there is a directed edge from variable $X$ to variable $Y$ if $X$ is a direct cause of $Y$. From the observational distribution, it can be shown that the true underlying causal graph can be recovered up to a Markov equivalence class (MEC) \cite{koller2009probabilistic}. There are two main approaches for recovering an MEC: constraint-based and score-based approaches. In the constraint-based approach, the MEC is identified by performing sufficient number of conditional independence (CI) tests over the observational distribution. PC \cite{spirtes2000causation} is a well-known algorithm for performing such CI tests in an efficient manner. PC algorithm runs in polynomial time to recover MEC if the maximum degree of causal graph is bounded by a constant. In the score-based approaches, the goal is to find the class of graphs maximizing a likelihood based score. Greedy equivalence search (GES) \cite{chickering2002optimal}  is one of the main score-based algorithms which reconstructs MEC by adding edges in a greedy manner.

As we mentioned above, without further assumption on the causal model, one can recover the causal graph up to an MEC. In order to uniquely recover the causal graph, we need to consider further assumptions on the causal mechanisms. For instance, if the causal mechanisms are non-linear and exogenous noises are additive, then the causal structure can be identified uniquely \cite{hoyer2008nonlinear}. Moreover, if the causal mechansims are linear, we can still recover the causal graph uniquely if the additive exogenous noises are non-Gaussian \cite{shimizu2006linear}. This assumption on the model is commonly called linear non-Gaussian acyclic model (LiNGAM) \cite{shimizu2006linear}. In ~\cite{shimizu2006linear}, an algorithm based on independent component analysis (ICA), commonly called ICA-LiNGAM, has been proposed which recovers the true causal graph under LiNGAM model. Later, a regression based method, called DirectLiNGAM ~\cite{shimizu2011directlingam}, has been presented to mitigate issues in using ICA algorithm. DirectLiNGAM algorithm has two main steps. In the first step, a causal order is obtained over the variables in the system. To do so, we compare any pair of variables like $X$ and $Y$, by regressing $Y$ on $X$ and checking whether the residual is independent of $Y$. A score is computed to measure the amount of dependency ~\cite{hyvarinen2013pairwise}. Afterwards, we select a variable that is most independent of its residuals, i.e., having minimum score among remaining variables and then append it to the causal order. We call this variable in each iteration as the root variable. Next, we remove this variable from the system by regressing it out and repeat the same procedure above until no variable is remained. After obtaining the causal order, in the second step, we perform multiple linear regressions based on the causal order in order to recover the underlying causal graph.


The executions of constraint-based or score-based algorithms might become too time-consuming as the number of variables increases in the system \cite{zarebavani2019cupc}. There have been some recent efforts to accelerate causal structure learning algorithms on multi-core machines. 
In the constraint-based approach,  in~\cite{le2015fast}, Le et al. implemented a parallel  version for a variant of PC algorithm (called PC-stable) on multi-core CPUs which reduces the runtime by an order of magnitude. Madsen et al. \cite{madsen2017parallel} proposed a method to perform conditional independence tests in parallel for PC algorithm. For the case of using GPU hardware, Schmidt et al. \cite{schmidt2018order} proposed a method to parallelize a small part of PC-stable algorithm. In \cite{zarebavani2019cupc}, Zare et al. proposed a GPU-based parallel algorithm for accelerating the whole PC-stable algorithm. The proposed algorithm parallelizes conditional independence tests over the pairs of variables or the conditional sets. Experimental results showed a significant speedup ratio up to 4000 in various real dataset. In \cite{schmidt2019out}, Schmidt et al. devised an out-of-core solution for accelerating PC-stable in order to handle extremely high-dimensional settings. Later, for discrete data, Hagedorn and Huegle \cite{hagedorn2021gpu} proposed a parallel PC algorithm on GPU for learning causal structure. Recently, Srivastava et al. \cite{srivastava2020parallel} presented a parallel framework to learn causal structures based on discovering Markov Blankets.

In score-based approach, Ramsey et al. \cite{ramsey2017million} proposed fast GES algorithm which accelerates updating score by caching scores of previous steps. They also implemented a parallel version of it on multi-core CPUs. Furthermore, there is a recent parallel solution for other search algorithms in the score based approach \cite{lee2019parallel}. %\blue{and estimation of distribution \cite{morigpu}}.

%\blue{The mentioned thesis was not quite relevant to our work, because it focused more on the CHC algorithm modification. Instead, I found this article that parallels the estimation of distribution algorithm (which they said is similar to genetic algorithms). Still, I am not sure it is a good paper to cite because there was not much information about its journal (International Journal of Informatics Society), and no one has not cited it yet. I added the paper to the Previous Works folder. "GPU Acceleration of EDA-based Algorithms to Learn Bayesian Networks"}

%\textbf{Multi-core CPU}:
%
%\cite{le2015fast} : A Fast PC Algorithm for High Dimensional Causal Discovery with Multi-Core PCs
%
%\cite{madsen2017parallel} : A parallel algorithm for Bayesian network structure learning from large data sets -- latest work of Madsen. Madsen has the first two parallel implementations for PC. As we discussed, we are going to just mention the latest. 

%\textbf{GES}:
%
%\cite{ramsey2017million} : A million variables and more: the Fast Greedy Equivalence Search algorithm for learning high-dimensional graphical causal models, with an application to functional magnetic resonance images -- fast GES, it also has some modifications


%\textbf{GPU}:
%
%schmidt ...
%\cite{schmidt2018order} : Order-independent constraint-based causal structure learning for Gaussian distribution models using GPUs -//- GPU before cuPC
%
%\cite{schmidt2019out} : Out-of-Core GPU-Accelerated Causal Structure Learning
%-//- using two GPU for speedup
%
%\cite{zarebavani2019cupc} : cuPC: Cuda-based parallel pc algorithm for causal structure learning on gpu
%
%\cite{hagedorn2021gpu} : GPU-Accelerated Constraint-Based Causal Structure Learning for Discrete Data -//- German research team's latest work (other authors) they compared their work with cuPC too

%\textbf{Simulated Annealing}:
%
%\cite{lee2019parallel} : Parallel simulated annealing with a greedy algorithm for Bayesian network structure learning

%\textbf{Hybrid}:
%
%\cite{tang2019penbayes} : PEnBayes: A Multi-Layered Ensemble Approach for Learning Bayesian Network Structure from Big Data
%
%\cite{guo2020scalable} : Scalable and Hybrid Ensemble-Based Causality Discovery

%\textbf{Markov Blanket}:
%
%\cite{srivastava2020parallel} : A parallel framework for constraint-based bayesian network learning via markov blanket discovery -//- 3 algorithms Grow-Shrink, Incremental Association MB (IAMB) , Interleaved IAMB.
%previsous works are the works for parallelizing MMHC(2006) PCMB(2007)


%\textbf{Framework}:
%A framework for Causal Structure Learning, testing PC (used cuPC and other implementations...)
%\cite{huegle2021mpcsl} : MPCSL - A Modular Pipeline for Causal Structure Learning



There are some recent studies with the main focus on evaluating the performance of causal structure learning algorithms in recovering the true underlying causal graph \cite{scutari2018learns,heinze2018causal}. It has been shown that LiNGAM algorithm has comparable or better performance than most existing methods and it is more suitable for high dimensional settings \cite{heinze2018causal}. Unfortunately, the runtimes of both variants of LiNGAM algorithm (ICA-LiNGAM or DirectLiNGAM) grow significantly as the number of variables increases. Thus, the current sequential implementations cannot be utilized for dataset with large number of variables. To the best of our knowledge, there is no previous parallel implementation of LiNGAM algorithm. In this paper, we propose a parallel algorithm, which we call ParaLiNGAM, for learning causal structure based on DirectLiNGAM algorithm. Our experiments show that the first step of DirectLiNGAM is computationally intensive and we focus on accelerating this step in this paper. Similar to DirectLiNGAM, we obtain the causal order in a number of iterations sequentially while in each iteration, we parallelize the process of finding the root variable.  
The main contributions of the paper are given as follows: 

\begin{itemize}
\item 
We propose a threshold mechanism in order to reduce the number of comparisons in each iteration. In this mechanism, we consider an upper limit on the score of root variable and whenever a variable exceeds this limit, we do not perform further comparisons corresponding with that variable. Our experiments show that the threshold mechanism can save up to $93.1\%$ comparisons that we have in DirectLiNGAM.
\item When we compare variable $X$ with $Y$, a part of computation is similar to the case that we are comparing $Y$ with $X$ in the reverse direction. Thanks to this observation, we employ a messaging mechanism in order to avoid performing redundant computations which reduces runtimes by a factor of about two.
\item We derive the mathematical formulations for normalizing and also regression which are frequently utilized in DirectLiNGAM algorithm. These mathematical formulations enable us to reduce the runtime and use the memory more efficiently.   
% for the task of comparison which results in reducing the frequency of reading  samples from the memory. 


 %Mathematics simplifications, storage (memory usage) is more efficient for variables ... which helps to fit in GPU
%\item Comparison Balance (also lock)
%\item 
%\item shared memory .. (not sure) Code
%\item Two strategies 
\item We evaluate ParaLiNGAM on various synthetic and real data. Experimental results show that the proposed algorithm can reduce runtime of DirectLiNGAM significantly by a factor up to $4657$.
\end{itemize}


 

The rest of this paper is organized as follows. In Section \ref{sec:prelim}, we review some preliminaries on structural equal models, LiNGAM model, and DirectLiNGAM algorithm. In Section \ref{sec:alg}, we present  ParaLiNGAM algorithm for learning causal structures in LiNGAM model. We provide some implementation details in Section \ref{sec:alg2}. We evaluate the performance of ParaLiNGAM algorithm in Section \ref{sec:exp}. Finally, we conclude the paper in Section \ref{sec:conc}.


==> LiNGAM(A23) - arXiv/prelim.tex <==
\section{Preliminaries}
\label{sec:prelim}

\subsection{Structural equation models}
\label{sec:prelim:sem}
Structural equation models (SEMs) are mathematical models that can be used to describe the data-generating process and causal relations of variables \cite{bollen1989structural, pearl2000models}. In particular, SEMs consists of a collection of $p$ equations where $p$ is the number of variables in the system. The causal mechanism of assigning values to the variable $X_j$, $1\leq j \leq p$, can be written as follows:
\begin{equation}
	X_j= f_j(PA_j, N_j),
\end{equation}
where $PA_j$ are called parents of $X_j$ and have direct cause on it. Moreover, $N_j$ is the exogenous noise corresponding to variable $X_j$. Exogenous noises are generated outside of the model and their data-generation processes are not modeled in the SEM.
We can represent causal relationships among the variables in an SEM by a directed graph where there is a directed edge from $X_i$ to $X_j$ if  $X_i \in PA_j$.
\begin{Example}
Consider the following SEM: 
\begin{figure}[tp]
	\centering
	\includegraphics[width = 0.45 \columnwidth]{fig/Casuse_effect}	
	\caption{Example of an SEM.}
	\label{fig:pre:SEM} 
\end{figure}
\begin{equation}
	\begin{gathered}
		X_3 = N_3, \\
		X_5 = f_5(X_3, N_5), \\
		X_1 = f_1(X_5, N_1), \\
		X_4 = f_4(X_1, N_4), \\
		X_2 = f_2(X_3, X_4, N_2),
	\end{gathered}
	\label{eq:sem}
\end{equation}
where the corresponding causal graph is illustrated in \mRefFig{fig:pre:SEM}. As can be seen, there is a directed edge from a direct cause to its effect. For instance, $X_3$ is the direct cause of $X_5$ and there is a directed edge from $X_3$ to $X_5$. 

%which shows data-generation process of $x_i, i\in{1,...,5}$ variables. In this SEM, $e_i$ are known as exogenous variables whose values are generated outside of the model, and their data-generation process is not modeled. In contrast, variables whose values are generated inside the model by other variables and functions($x_i$) are known as endogenous variables. We can use these models to describe a causal structure, in which every edge shows a cause-effect relation. For example $x_3$ is cause and $x_5$ is effect.
% for further expansion we can use "each SEM consists of 4 parts ..." or "Interventions in SEMs ..."
\label{ex:base}
\end{Example}

% Consider the SEM illustrated in \mRefFig{fig:pre:SEM}, we can write
%\begin{figure}[tp]
%	\centering
%	\includegraphics[width = \columnwidth]{fig/SEM}	
%	\caption{Example of an SEM} 
%	\label{fig:pre:SEM} 
%\end{figure}
%\begin{equation}
%	\begin{gathered}
%	x_3 = e_3 \\
%	x_5 = f_1(x_3, e_5) \\
%	x_1 = f_2(x_5, e_1) \\
%	%TODO Saleh is it better to write it as f_2(x_3, x_5, e_1)?
%	x_4 = f_3(x_1, e_4) \\
%	x_2 = f_4(x_3, x_4, e_2),
%	\end{gathered}
%\label{eq:sem}
%\end{equation}
%which shows data-generation process of $x_i, i\in{1,...,5}$ variables. In this SEM, $e_i$ are known as exogenous variables whose values are generated outside of the model, and their data-generation process is not modeled. In contrast, variables whose values are generated inside the model by other variables and functions($x_i$) are known as endogenous variables. We can use these models to describe a causal structure, in which every edge shows a cause-effect relation. For example $x_3$ is cause and $x_5$ is effect.
%% for further expansion we can use "each SEM consists of 4 parts ..." or "Interventions in SEMs ..."


\subsection{Linear Non-Gaussian Acyclic Model (LiNGAM)}
 One of the common assumption in the literature of causality is that the causal relations between variables are acyclic, i.e., the corresponding causal graph is a \textbf{directed acyclic graph} (\textbf{DAG})\footnote{A directed acyclic graph is a graph whose edges are all directed and there is no directed
cycle in the graph.}. By this assumption, there is always a \textbf{causal order} of variables $X_i$, $i\in\{1,\dotsc,p\}$, in the DAG so that no latter variable in the causal order has a direct path to any earlier variable. We denote the position of each variable $X_i$ in the causal order by $k(i)$. For instance, for the causal graph in \mRefFig{fig:pre:SEM}, $k=[3,5,1,4,2]$
 is a causal order.

 %which is $k = [x_3, x_5, x_1, x_4, x_2]$ in previous example.
 
As an additional assumption, one can consider that the functional relations of variables are linear. Thus, the model can be reformulated as follows:
\begin{equation}
	X_i = \sum_{k(j)<k(i)}b_{ij}X_{j} + N_i,
\label{eq:base_linear}
\end{equation}
where $b_{ij}$ is the causal strength representing magnitude of direct causation from $X_j$ to $X_i$. Furthermore, it is assumed that the exogenous noises have zero mean, non-zero variance, and are independent of each other (i.e., no latent confounder is in the system). We can rewrite Eq. \ref{eq:base_linear} in the matrix form as follows:
\begin{equation}
X = BX + N,
\label{eq:base_mat}
\end{equation}
where $X$ and $N$ are $p$-dimensional random vectors, and $B$ is a $p \times p$ matrix of causal strengths. For instance, the SEM of \mRefFig{fig:pre:SEM} can be written as follows:
\begin{equation}
\begin{bmatrix}
X_1 \\ X_2 \\ X_3 \\ X_4 \\ X_5
\end{bmatrix}
=
\begin{bmatrix}
0 & 0 & 0 & 0 & 3 \\
0 & 0 & 6 & -3 & 0 \\
0 & 0 & 0 & 0 & 0 \\
4 & 0 & 0 & 0 & 0 \\
0 & 0 & 5 & 0 & 0 \\
\end{bmatrix}
\begin{bmatrix}
X_1 \\ X_2 \\ X_3 \\ X_4 \\ X_5
\end{bmatrix}
+
\begin{bmatrix}
N_1 \\ N_2 \\ N_3 \\ N_4 \\ N_5
\end{bmatrix}
,
\label{eq:base_mat_ex}
\end{equation}
where zero entries of $B$ show the absence of directed edges. It can be shown that a simultaneous permutations of rows and columns of matrix $B$ according to a causal order can convert it to a \textbf{strictly lower triangular} matrix, due to the acyclicity assumption \cite{bollen1989structural}.
In the example in \mRefFig{fig:pre:SEM}, we can rewrite equations in the following form to make the matrix $B$ strictly lower triangular:
\begin{equation}
\begin{bmatrix}
X_3 \\ X_5 \\ X_1 \\ X_4 \\ X_2
\end{bmatrix}
=
\begin{bmatrix}
0 & 0 & 0 & 0 & 0 \\
5 & 0 & 0 & 0 & 0 \\
0 & 3 & 0 & 0 & 0 \\
0 & 0 & 4 & 0 & 0 \\
6 & 0 & 0 & -3 & 0 \\
\end{bmatrix}
\begin{bmatrix}
X_3 \\ X_5 \\ X_1 \\ X_4 \\ X_2
\end{bmatrix}
+
\begin{bmatrix}
N_3 \\ N_5 \\ N_1 \\ N_4 \\ N_2
\end{bmatrix}
.
\label{eq:base_mat_ex_prder}
\end{equation}

% we can talk about the insufficiency of Gaussian distribution in determining full structure.
 It can be shown that the causal structure cannot be recovered uniquely if the distributions of exogenous noises are Gaussian ~\cite{pearl2000models}.
However, in ~\cite{shimizu2006linear}, it has been proved that the model can be fully identified from observational data if all the exogenous noises are non-Gaussian. They called the non-Gaussian version of the linear acyclic SEM,  \textbf{Linear} \textbf{Non-Gaussian} \textbf{Acyclic Model} (\textbf{LiNGAM}). In the rest of this paper, we assume the model of data generation obeys the assumptions in LiNGAM.
 %, is proposed and proved that can identify the model completely, only based on the observed data.

\subsection{Causal Structure Learning Algorithms for LiNGAM}
\label{sec:baseLiNGAM}
ICA-LiNGAM ~\cite{shimizu2006linear} was the first algorithm for the LiNGAM model, which applies an independent component analysis (ICA) algorithm to observed data and try to find the best strictly lower triangular matrix for $B$ that fits the observed data. This algorithm is fast due to well-developed ICA techniques. However, the algorithm has several drawbacks, e.g., getting stuck in local optimal, scale-dependent calculations, and usually estimating dense graph even for sparse ground truth causal graphs~\cite{shimizu2011directlingam}.
% also we can talk about the 2008 log likelihood alg.

\textbf{DirectLiNGAM} was proposed in~\cite{shimizu2011directlingam}, in order to resolve ICA-LiNGAM's issues and converges to an acceptable approximation of matrix $B$ in a fixed number of steps. 
Also, we can provide prior knowledge to the algorithm, which can improve the performance of recovering the correct model. However, computation cost of DirectLiNGAM is more than ICA-LiNGAM, and it cannot be applied on large graphs\cite{shimizu2011directlingam}.
%\red{Do we have experimental results to show it or cite a paper?} \blue{In DirectLiNGAM, there is a Computational complexity section (Section 3.3), which discusses this matter. Moreover, in simulations of the paper (Section 4), the runtime of both algorithms is compared. So, we can cite \cite{shimizu2011directlingam} again at the end of paragraph.}


DirectLiNGAM algorithm consists of two main steps: In the first step, the causal order of variables is estimated by repeatedly searching for a root in the remaining graph and regressing out its effect on other variables. In the second step, causal strengths are estimated by using some conventional covariance-based regression according to the recovered causal order~\cite{shimizu2011directlingam}. Experimental results show that the second step is fairly fast since we are only performing linear regressions. However, the first step is computationally intensive and we focus on accelerating this part in this paper. 

%Details of the first step are described in the following.

\begin{algorithm}[tp]
	\begin{algorithmic}[1]
		\Input $\mathcal{X}$
		\Output $K$
		%
		\State $U =\{1,\cdots, p\}$ 
		\State $K=\emptyset$
		\Repeat
			\State $root = FindRoot(\mathcal{X}, U)$
			\State Append $root$ to $K$
			\State Remove $root$ from $U$
			\State $\mathcal{X} = RegressRoot(\mathcal{X}, U, root)$
		\Until{$U$ is not empty}
		\State Estimate causal strengths $B$ from $K$
	\end{algorithmic}
	\caption{DirectLiNGAM} 
	\label{alg:baseLiNGAM}
\end{algorithm}


The description of DirectLiNGAM algorithm is given in \mRefAlg{alg:baseLiNGAM}. The input of the algorithm is matrix $[\mathcal{X}]_{p\times n}$
whose $i$-th row, $x_i$, contains $n$ samples from variable $X_i$.
 %is set of observed variables $x_i$, $i\in\{1,\dotsc,p\}$ which one each of them has $n$ samples.
The output of algorithm is $K$, a causal order list of variables. First, we initialize $U$ by a list of all variables' indecies and set $K$ to an empty list (lines $1-2$). Next, $K$ is going to be filled with variables from $U$ using a comparison between variables to form a causal order. Recovering a causal order takes $p$ (size of $U$) iterations. In each iteration, the most independent variable in $U$ ($root$ of that iteration) is determined by the $FindRoot$ function. Then the $root$ moves from $U$ to $K$. Next, the data of remaining variables in $U$ are updated by regressing them on the root ($RegressRoot$ function), which has been shown that it preserves correct causal orders in the remaining part ~\cite{shimizu2011directlingam}. Finally, the matrix B is recovered from the causal order in $K$s using conventional covariance-based regression methods.

%\red{Somewhere we need to define our notations for small and capital letters.} \blue{$X, x$ ?}

% This is for prior knowledge extension
%\begin{algorithm}[tp]
%	\begin{algorithmic}[1]
%		\Input $X, U$
%		\Output $root$
%		%
%		\State $U_c, V_j = SearchCandidate(U)$
%		\If {$U$ has only one element}
%			\State return the element
%		\EndIf
%		%\State $Scores = \emptyset$ 
%		\For {$i$ in $U_c$}
%			\State $Score = 0$
%			\For {$j$ in $U\backslash\{i\}$}
%				\State $Normalize(x_i)$
%				\State $Normalize(x_j)$
%				\If {$i$ in $V_j$ and $j$ in $U_c$}
%					$r_i^{(j)} = x_i$
%				\Else {}
%					$r_i^{(j)} =  Regress(x_i, x_j)$
%				\EndIf
%				\If {$j$ in $V_j$ and $i$ in $U_c$} $r_j^{(i)} = x_j$
%				\Else {} $r_j^{(i)} =  Regress(x_j, x_i)$
%				\EndIf
%				\State $Normalize(r_i^{(j)})$
%				\State $Normalize(r_j^{(i)})$
%				\State $Score += \min\{0, Diff\_MI(x_i, x_j, r_i^{(j)}, r_j^{(i)})\}^2$
%			\EndFor
%			\State Store $-Score$
%		\EndFor
%		\State $root=$ element of $U_c$ with maximum $Score$
%	\end{algorithmic}
%	\caption{$FindRoot$} 
%	\label{alg:baseLiNGAM_FR}
%\end{algorithm}

\begin{algorithm}[tp]
	\begin{algorithmic}[1]
		\Input $\mathcal{X}, U$
		\Output $root$
		%
		\If {$U$ has only one element}
			\State return the element
		\EndIf
		\State $\mathcal{S} = [\textbf{0}]_{|U|}$ 
		\For {$i$ in $U$}
			\For {$j$ in $U\backslash\{i\}$}
				\State $Normalize(x_i)$
				\State $Normalize(x_j)$
%				\State $\mathcal{S} += Compare(x_i, x_j)$
 			
% 				// Start of $Compare$ Function
				\State $r_i^{(j)} =  Regress(x_i, x_j)$
				\State $r_j^{(i)} =  Regress(x_j, x_i)$
				\State $Normalize(r_i^{(j)})$
				\State $Normalize(r_j^{(i)})$
				\State $\mathcal{S}[i] += \min\{0, \mTest(x_i, x_j, r_i^{(j)}, r_j^{(i)})\}^2$
			\EndFor
		\EndFor
		\State $root=$ $U[arg\min(Scores)]$
	\end{algorithmic}
	\caption{$FindRoot$} 
	\label{alg:baseLiNGAM_FR}
\end{algorithm}


The purpose of $FindRoot$ function (see \mRefAlg{alg:baseLiNGAM_FR}) is to find most independent variable from its residuals by comparing all pairs of variables given in $U$. Each variable in $U$ has a score with initial value of zero and all of them are stored in an array called $\mathcal{S}$ (line $4$).
First, samples of each variable are normalized. Next, each variable $X_i$ is regressed on any other variable like $X_j$ in $U$. Afterwards, the regressed values are normalized. Finally, an independence test $\mTest$ is performed and its result is added to a score of variable $X_i$. In ~\cite{hyvarinen2013pairwise}, a likelihood ratio test is proposed that assigns a real number to the pair of variables:
\begin{equation}
%\!\begin{multlined}[t]
\mTest(x_i, x_j, r_i^{(j)}, r_j^{(i)}) = H(x_j) + H(r_i^{(j)}) - H(x_i) - H(r_j^{(i)}),
%\end{multlined}
\label{eq:Itest}
\end{equation}
where $H$ is differential entropy, which can be approximated by computationally simple function as follows ~\cite{hyvarinen2013pairwise, hyvarinen1998analysis}:


%\blue{(I think I should cite Hyvarinen's earlier paper \cite{hyvarinen1998analysis} in which he mentioned this formula in the first place instead. right?)}
\begin{equation}
\!\begin{multlined}[t]
\hat{H}(u) = H(v) - k_1[E\{\log\cosh(u)\}- \beta]^2 \\
 - k_2[E\{u\exp(-u^2/2)\}]^2.
\end{multlined}
\label{eq:HApp}
\end{equation}


In above equation, $H(v) = \frac{1}{2}(1 + \log2\pi)$ is the entropy of the standardized Gaussian distribution, and the other constants can be set to:
\begin{center}
$k_1 \approx 79.047,$\\
$k_2 \approx 7.4129,$\\
$\beta \approx 0.37457.$\\
\end{center}

% First, samples of each variable is normalized and then regressed on each other. Next, the regressed values are normalized too. Finally, an independence test $\mTest$ is used to compare variables. In ~\cite{hyvarinen2013pairwise}, a likelihood ratio test is proposed that assigns a real number to the pair of variables.
%This method has better results and less computation complexity compared to previous methods ~\cite{shimizu2011directlingam} 
A positive/negative value of $\mTest$ indicates the independence/dependence of that variable compared to the other one. For aggregating score for each variable and determining total independence of a variable from others, only the amount of dependence is considered. 
In other words, in this method, only negative value of $I$ are considered and its square is added to the score.
The variable with minimum score is selected as the root variable. 
Please note that we consider lines $9-13$ as \textbf{$Compare$} function and use this as the based function for comparing two variables in next sections.

 %to the variables, and the maximum value of final score for a variable($root$'s $Score$) is zero (case that the variable is independent of all of the others).

%\begin{figure}[tp]
%	\centering
%	\includegraphics[width = \columnwidth]{fig/example}	
%	\caption{An example of execution first two iterations of DirectLiNGAM algorithm. $r_i^{(j)}$ denotes the residual when $X_i$ is regressed on $X_j$. The last column shows the scores corresponding to the variables.} 
%	\label{fig:pre:ex} 
%\end{figure}

%
%\begin{Example}
%\label{ex:pre}
%	\mRefFig{fig:pre:ex} illustrates score of variables in the execution of the first two iterations for the SEM given in \mRefEx{ex:base}. 
%	In the first iteration, score of $X_1$ is calculated by comparing with the other variables. The value of test would be zero when it is compared with $X_2$ and $X_4$ due to being independent of the residuals. Moreover, this variable is child/descendant  of $X_5$/$X_3$ which makes it dependent to the residuals and gets a positive score. Next, score of $X_2$ is calculated, and all of the scores are non-zero. Because it is descendant of all other variables. While the score of $X_3$ is zero because it is the root of DAG and is independent of its residuals, when compared to all other variables. The score of $X_4$ and $X_5$ are calculated accordingly and $X_3$ is chosen as a root in the first iteration. Next, other variables are updated by regressing on $X_3$. In the second iteration, similar to the first iteration, all pairs of remaining variables in $U$ are compared and this time, $X_5$ is chosen as the root.
%\end{Example}



